Fair and Efficient Allocations Without Obvious Manipulations

We consider the fundamental problem of allocating a set of indivisible goods among strategic agents with additive valuation functions. It is well known that, in the absence of monetary transfers, Pareto efficient and truthful rules are dictatorial, while there is no deterministic truthful mechanism that allocates all items and achieves envy-freeness up to one item (EF1), even for the case of two agents. In this paper, we investigate the interplay of fairness and efficiency under a relaxation of truthfulness called non-obvious manipulability (NOM), recently proposed by Troyan and Morrill. We show that this relaxation allows us to bypass the aforementioned negative results in a very strong sense. Specifically, we prove that there are deterministic and EF1 algorithms that are not obviously manipulable, and the algorithm that maximizes utilitarian social welfare (the sum of agents' utilities), which is Pareto efficient but not dictatorial, is not obviously manipulable for $n \geq 3$ agents (but obviously manipulable for $n=2$ agents). At the same time, maximizing the egalitarian social welfare (the minimum of agents' utilities) or the Nash social welfare (the product of agents' utilities) is obviously manipulable for any number of agents and items. Our main result is an approximation preserving black-box reduction from the problem of designing EF1 and NOM mechanisms to the problem of designing EF1 algorithms. En route, we prove an interesting structural result about EF1 allocations, as well as new "best-of-both-worlds" results (for the problem without incentives), that might be of independent interest.

==> everything.tex <==
\subsection{Main result: fPO + EF1 + NOM}
\paritosh{To-do: 3. Remove notational inconsistency.}


As we discussed in Section~\ref{sec: intro}, a popular way to achieve fairness and efficiency simultaneously, for additive agents, is to compute the allocation which maximizes the Nash social welfare~\cite{caragiannis2019unreasonable}. However, as we've seen in Theorem~\ref{thm: MNW impossibility}, this rule is obviously manipulable. 
In this section we present a new $\NOM$ mechanism (Mechanism \ref{mechanism:NOM+PO+EF1}) that outputs $\fPO + \EFone$ allocations. Notably, Mechanism \ref{mechanism:NOM+PO+EF1} uses, as a black-box, any deterministic mechanism that outputs $\fPO + \EFone$ allocations; see, for e.g., \cite{garg2021fair}. That is, our proposed mechanism can also be viewed as a framework that converts any given $\fPO + \EFone$ mechanism into a $\NOM$ mechanism for $\fPO + \EFone$. Formally, the main result of this section is stated as the following theorem.

\begin{theorem}
\label{theorem:NOM+PO+EF1}
There exists a deterministic, not obviously manipulable mechanism that achieves fractional-Pareto efficiency and envy-freeness up to one item.
\end{theorem}

\alex{Attempt at more general theorem:
Given access to a deterministic algorithm $\mathcal{M}^*$ that (1) allocates every item $g \in \items$ to an agent that values it, if such an agent exists (not sure what this means beyond additive...), 

}

The above theorem is established by showing that Mechanism~\ref{mechanism:NOM+PO+EF1} is $\NOM$ and always outputs $\fPO + \EFone$ allocations.

\floatname{algorithm}{Mechanism}
\begin{algorithm}[!h]
\caption{\alex{fix}} \label{mechanism:NOM+PO+EF1}

%Input-Output
\textbf{Input:} Reported valuation of agents $(\bids_1, \bids_2, \ldots, \bids_n)$ where each $\bids_i \in \mathbb{R}_{\geq 0}^m$.\\
\textbf{Output:} $\PO + \EFone$ integral allocation $\alloc = (X_1, \ldots, X_n)$ 
%Pseudo code
  \begin{algorithmic}[1]
  		%Initialization
  		\STATE Remove all goods that are not wanted by any agent: $\items \gets \items \setminus \{ g \in \items | v_{i,g} = 0, \forall i \in \agents \} $
  		\STATE \textbf{Set} $D_i \gets \{j \in \items \ | \ b_{i,j} > 0\}$ for each $i \in \agents$. %\COMMENT{$D_i$ is the set of goods having positive value for agent $i$, i.e., goods desired by agent $i \in [n]$.}
  		\STATE \textbf{Set} $\widehat{D}_i \gets \items \setminus \cup_{j\neq i} D_j$ for each $i \in \agents$.
		\STATE \textbf{Set} $R_i \gets 1$ if subsets $\{D_j\}^n_{j=1} \setminus \{D_i\}$ are pairwise disjoint; $0$ otherwise.  		
  		
  		\STATEx - - -\emph{Case $\rm{I}$} - - -
  		\IF{the subsets $\{D_j\}_{j=1}^n$ are pairwise disjoint}
  			\STATE \textbf{return} $(D_1, \ldots, D_n)$%\COMMENT{the returned allocation is $\PO + \EFone$}
  			
  		\STATEx - - -\emph{Case $\rm{II}$} - - -
  		\ELSIF{$\exists i \in \agents$ such that $R_i = 1$ and $R_j = 0$ for every $j \in \agents \setminus \{i\}$} \label{case2-begin}
  			
  			\IF{the allocation $(D_1, D_2, \ldots, \widehat{D}_i, \ldots, D_n)$ is $\EFone$}
  				\STATE \textbf{return} $(D_1, D_2, \ldots, \widehat{D}_i, \ldots, D_n)$ \label{case2-return1}
  			\ELSE
  				\STATE \textbf{return} $M(\bids_1, \bids_2, \ldots, \bids_n)$
  			\ENDIF \label{case2-end}
  			
  		
  		\STATEx - - -\emph{Case $\rm{III}$} - - -
  		\ELSIF{$\exists i,j \in \agents$ such that $i<j$ and $R_i = R_j = 1$, and $R_k =0$ for $k \in [n] \setminus \{i,j\}$} \label{case3-begin}
  			\IF{$\sum_{g \in D_i \cap D_j} v_{i,g} < \sum_{g \in D_i \cap D_j} v_{j,g}$} \alex{update to $v_i(D_i \cap D_j) < v_j(D_i \cap D_j)$ for submodular} \label{case3-tie-breaking:begin}
				\IF{$(D_1, \ldots, \widehat{D}_i, \ldots, D_j, \ldots, D_n)$ is $\EFone$} \label{case3-subcase1-if}
					\STATE \textbf{return} $(D_1, \ldots, \widehat{D}_i, \ldots, D_j, \ldots, D_n)$ \label{case3-subcase1-return}
				\ELSE
					\STATE \textbf{return} $M(\bids_1, \bids_2, \ldots, \bids_n)$
				\ENDIF  \label{case3-subcase1:end}		
  			\ELSE \label{case3-subcase2:begin}
				\IF{$(D_1, \ldots, D_i, \ldots, \widehat{D}_j, \ldots, D_n)$ is $\EFone$} 
					\STATE \textbf{return} $(D_1, \ldots, D_i, \ldots, \widehat{D}_j, \ldots, D_n)$
				\ELSE
					\STATE \textbf{return} $M(\bids_1, \bids_2, \ldots, \bids_n)$ 
				\ENDIF 
  			\ENDIF \label{case3-tie-breaking:end}
  			\tikzmark{bottom}
  		\STATEx - - -\emph{Case $\rm{IV}$} - - -
  		\ELSE
  			\STATE \textbf{return} $M(\bids_1, \bids_2, \ldots, \bids_n)$
  		\ENDIF
		\end{algorithmic}
\end{algorithm}

\paritosh{Describe the main idea behind the proof}\\

Let $\mathcal{M}^*$ be an arbitrary ... \alex{todo}

%Suppose the reported valuation of each agent $i \in [n]$ is $v_i \in \mathbb{R}_{\geq 0}^m$. 
\alex{For submodular, $D_i$ can be defined as the smallest set that gives $i$ her maximum utility.}
Given the reported valuations $\{\bids_i\}^n_{i=1}$,  Mechanism~\ref{mechanism:NOM+PO+EF1} considers, for each agent $i \in \agents$, the set of goods that are desired by her, $D_i \coloneqq \{g \in \items \ : \ b_{i,g} > 0\}$.
Let $\widehat{D}_i \coloneqq \items \setminus \cup_{j\neq i} D_j$ be the set of items remaining after removing all goods desired by agents other than $i$. Finally, let $R_i$, for each agent $i \in \agents$, be the indicator for the event that the subsets $( \{D_j\}_{j \in \agents}) \setminus D_i$ are pairwise disjoint, i.e. $R_i = 1$ iff $( \{D_j\}_{j \in \agents}) \setminus D_i$ are pairwise disjoint, and $R_i = 0$ otherwise. Note that the $R_i$s can be easily computed in polynomial time, given the reports. 
Mechanism~\ref{mechanism:NOM+PO+EF1} sequentially considers four cases based on the sets $\{D_j\}^n_{j=1}$ and the values $\{R_j\}^n_{j=1}$:

\begin{description}
\item[\emph{Case \rm{I}}:] The sets $\{D_j\}^n_{j=1}$ are pairwise disjoint (equivalently, $R_i = 1$ for all $i \in \agents$). In this case, the mechanism allocates the bundle $D_j$ to agent $j$ for each agent $j \in \agents$.
\item[\emph{Case \rm{II}}:] $R_i = 1$ for exactly one agent $i \in \agents$. This can occur if $D_i$ intersects with two or more $D_j$s (and these are the only intersections). In this case, if allocating the bundle $\widehat{D}_i$ to agent $i$, and the bundle $D_j$ to each agent $j \in \agents$, $j \neq i$ is $\EFone$, then Mechanism~\ref{mechanism:NOM+PO+EF1} returns this allocation (note that, by definition, this is a feasible allocation). Otherwise, if this allocation is not $\EFone$, Mechanism~\ref{mechanism:NOM+PO+EF1} returns the allocation of the blackbox mechanism $\mathcal{M}^*$ for the given valuation profile.
\item[\emph{Case \rm{III}}:] There are exactly two agents $i,j \in \agents$ such that $R_i = R_j = 1$. Note that the only way this is possible is if $D_i$, $D_j$ intersect each other and any other pair of subsets $D_k, D_l$ where $\{k,l\} \neq \{i,j\}$, are disjoint. In this case, Mechanism~\ref{mechanism:NOM+PO+EF1} considers whether the set of goods $D_i \cap D_j$ are valued more by agent $i$ or agent $j$; each of these two subcases are similar to \emph{Case \rm{II}}, see Lines \ref{case3-tie-breaking:begin}-\ref{case3-tie-breaking:end}.
\item[\emph{Case \rm{IV}}:] None of the previous cases holds (equivalently, $R_i = 0$ for all $i \in \agents$). In this case, Mechanism~\ref{mechanism:NOM+PO+EF1} simply returns the allocation of the blackbox mechanism $\mathcal{M}^*$ for the given valuation profile.
\end{description}


%In \emph{Case \rm{I}}, the set of goods desired by agent $\{D_j\}^n_{j=1}$ are pairwise disjoint, and the mechanism allocates the bundle $D_j$ to agent $j$ for each agent $j \in \agents$. 
%Otherwise, in \emph{Case \rm{II}}, there is a single agent $i \in \agents$ such that $R_i = 1$. Note that, the conditions corresponding to these cases are checked sequentially, as a consequence, in cases other than \emph{Case \rm{I}}, the sets $\{D_j\}^n_{j=1}$ are not pairwise disjoint. Thus, in \emph{Case \rm{II}} the subsets $\{D_j\}^n_{j=1}$ are not pairwise disjoint and there is one agent $i \in \agents$ such that $R_i = 1$, i.e., the subsets $\{D_j\}^n_{j=1} \setminus \{D_i\}$ are pairwise disjoint. In this case, if the allocation $(D_1, D_2, \ldots, \widehat{D}_i, \ldots, D_n)$ is $\EFone$ then the mechanism $\widehat{M}$ returns it, otherwise it return the allocation that mechanism $M$ (the blackbox mechanism for $\PO+\EFone$) would return for the given valuations. 
%In \emph{Case \rm{III}}, there are exactly two agents $i,j \in \agents$ having $R_i = R_j = 1$, and the subsets $\{D_j\}^n_{j=1}$ are not pairwise disjoint. Note that, this can happen only if the subsets $D_i$, $D_j$ intersect each other and any other pair of subsets $D_k, D_l$ where $\{k,l\} \neq \{i,j\}$ are disjoint. Here, the mechanism considers two subcases based on whether the set of goods $D_i \cap D_j$ are valued more by agent $i$ or agent $j$; each of these two subcases are similar to \emph{Case \rm{II}}, see Lines \ref{case3-tie-breaking:begin}-\ref{case3-tie-breaking:end}. Finally, in \emph{Case \rm{IV}}, the mechanism simply returns the allocation that the blackbox mechanism $M$ would output for the given valuation profile.

Towards establishing our main result, Theorem \ref{theorem:NOM+PO+EF1}, we begin by proving the following three supporting lemmas. In particular, the following lemma (Lemma \ref{lemma:PO+EF1}) shows that Mechanism~\ref{mechanism:NOM+PO+EF1} always outputs $\fPO$ and $\EFone$ allocations.

\begin{lemma}
\label{lemma:PO+EF1}
Mechanism~\ref{mechanism:NOM+PO+EF1} always outputs an allocation that is $\EFone$ and fractionally Pareto efficient.
\end{lemma}
\begin{proof}
First, notice that if all agents $j$ receive the bundle $D_j$ (as in case \rm{I}), the allocation is fractionally Pareto efficient and envy-free (and therefore $\EFone$). If all agents $j$ receive the bundle $D_j$, with the possible exception of a single agent $i$ that receives $\widehat{D}_i$, then the allocation is fractionally Pareto efficient, since everyone except $i$ gets the maximum possible utility \alex{for submodular, we would add here ``using the smallest possible set''}, and therefore $i$ cannot improve her utility without hurting another agent. This allocation is considered in cases \rm{II} and \rm{III} (if $\mathcal{M}^*$ is not called), and it is the output of Mechanism~\ref{mechanism:NOM+PO+EF1} if it is also $\EFone$, and therefore both properties are satisfied. Finally, in the remaining cases (if the aforementioned allocation is not $\EFone$, or we are in case \rm{IV}) Mechanism~\ref{mechanism:NOM+PO+EF1} returns the allocation of the blackbox mechanism $\mathcal{M}^*$, which satisfies the two properties by definition.
\end{proof}
%We prove that the mechanism $\widehat{M}$ returns $\PO + \EFone$ allocations in each of the four cases.

%\noindent
%\emph{Case \rm{I}}: The set of desired goods for all agents, $\{D_j\}^n_{i=1}$, are pairwise disjoint. Here, the mechanism $\widehat{M}$ returns the allocation $(\widehat{D}_1, D_2, \ldots, D_n)$. Since the subsets $\{D_j\}^n_{i=1}$ are pairwise disjoint, the bundle $\widehat{D}_1 = \items \setminus \cup_{j\neq i} D_j = D_i \cup \big( \items \setminus \cup^n_{j=1} D_j \big) \supseteq D_i$. Thus, in the allocation $(\widehat{D}_1, D_2, \ldots, D_n)$, each agent is getting all the goods that they desire, such an allocation is both $\PO + \EFone$.

%\noindent
%\emph{Case \rm{II}}: The boolean value $R_i = 1$ for exactly one agent $i \in \agents$. In this case, the mechanism $\widehat{M}$ checks whether the allocation $\Alloc = (D_1, D_2, \ldots, \widehat{D}_i, \ldots, D_n)$ is $\EFone$. If the allocation $\Alloc$ is $\EFone$, then $\widehat{M}$ returns $\Alloc$. Note that, allocation $\Alloc$ is also $\PO$ because every agent $j \in \agents \setminus \{i\}$ is getting all the goods they desire, i.e., there utility cannot be improved, and in order to improve agent $i$'s utility we must decrease the utility of some other agent $j \in \agents \setminus \{i\}$; hence the allocation $\Alloc$ is $\PO$. Therefore, if the allocation $\Alloc$ is $\EFone$, then the mechanism returns allocation $\Alloc$ which is $\EFone$ as well as $\PO$. Otherwise if the allocation $\Alloc$ is not $\EFone$, then the mechanism $\widehat{M}$ simply returns the $\PO + \EFone$ allocation that the mechanism $M$ returns.

%\noindent
%\emph{Case \rm{III}}: There are two agents $i,j \in \agents$ such that $R_i = R_j = 1$, and $R_k = 0$ for any other agent $k \in \agents \setminus \{i,j\}$. This can happen only if the subsets $D_i$ and $D_j$ intersect each other and no other pair of subsets in $\{D_k\}^n_{k=1}$ are intersecting. In this case, the mechanism $\widehat{M}$ considers two subcases based on whether the bundle $D_i \cap D_j$ is valued more by agent $i$ or agent $j$. In the first subcase, when agent $j$ values $D_i \cap D_j$ more than agent $i$ (Lines \ref{case3-tie-breaking:begin}-\ref{case3-subcase1:end}), either the mechanism $\widehat{M}$ outputs an $\EFone$ allocation $(D_1, \ldots, \widehat{D}_i, \ldots, D_j, \ldots, D_n)$ or uses the blackbox mechanism $M$ to compute a $\PO + \EFone$ allocation. Note that, the $\EFone$ allocation $(D_1, \ldots, \widehat{D}_i, \ldots, D_j, \ldots, D_n)$ will also be $\PO$ because every agent except agent $i$ is getting all their desired goods (thus their utility cannot be improved) and in order to improve the utility of agent $i$ we must decrease the utility of some other agent. Thus, in the first subcase $\widehat{M}$ outputs $\PO + \EFone$ allocations; the same argument also holds for the second subcase (Lines \ref{case3-subcase2:begin}-\ref{case3-tie-breaking:end}).

%\noindent
%\emph{Case \rm{IV}}: In this case, the mechanism $\widehat{M}$ returns the allocation that the mechanism $\widehat{M}$ returns %\end{proof}

The next lemma characterizes the set of allocations that Mechanism~\ref{mechanism:NOM+PO+EF1} could possibly return given the reported valuation of a particular agent. Before stating the lemma, we define some useful notation.
For any agent $i \in \agents$ and valuation vector $\values_i \in \mathbb{R}^m_{\geq 0}$, let $\EFone(i,\values_i)$ be the set of allocations $\Alloc = (A_1, \ldots, A_n)$ that are envy-free up to one item with respect to agent $i$ when her valuation vector is $\values_i$, and satisfy $v_{i,g} > 0$ for all $g \in A_i$: $\EFone(i,\values_i) = \{ \Alloc \in \Pi_n(\items) \ | \forall g \in A_i ~~ v_{i,g} > 0, \text{ and } \forall j \in \agents \text{ with } A_j \neq \emptyset, \values_i(A_i) \geq \values_i(A_j \setminus \{g\}) \text{ for some }g \in X_j\}$.
\alex{for submodular we would update the $v_{i,g} > 0$ to something that, again, expresses ``smallest''}


\begin{lemma}
\label{lemma:every-EF1-realized}
Given any agent $i \in \agents$ and valuation vector $\values_i \in \mathbb{R}^m_{\geq 0}$, for every allocation $\Alloc \in \EFone(i,v_i)$ there exists a set of valuations $\values_{-i}$ such that Mechanism~\ref{mechanism:NOM+PO+EF1} on input  $(\values_i, \values_{-i})$ outputs $\alloc$.
\end{lemma}

%\paritosh{Continue Cleanup from here}

\begin{proof}
\alex{I think here it's fine if all other agents are additive.}
Given the valuation vector $\values_i$ and an allocation $\Alloc = (A_1, A_2, \dots, A_n) \in \EFone(i,\values_i)$ we will construct valuations for the other agents, $\values_{-i}$, such that Mechanism~\ref{mechanism:NOM+PO+EF1} outputs $\alloc$ on input  $(\values_i, \values_{-i})$.  The constructed valuation vector of each agent $j \in (\agents \setminus \{i\})$ will be such that $v_{j,g} = 0$ for all $g \notin A_j$, and $v_{j,g} > 0$ for each good $g \in A_j$ (the precise value of $v_{j,g}$ will depend on how $D_i$ intersects with $A_j$). That is, for each agent $j \in (\agents \setminus \{i\})$, $D_j = A_j$. Therefore, by construction, the subsets $\{D_j\}^n_{j=1} \setminus \{D_i\}$ are pairwise disjoint, and therefore $R_i = 1$ (so, we are never in case $\rm{IV}$ of Mechanism~\ref{mechanism:NOM+PO+EF1}).
In the remainder of the proof, we describe the remaining details of the construction of $\values_{-i}$, by considering the three exhaustive cases, based on how many sets from $\Alloc \setminus A_i$ the set $D_i$ intersects.

The first case is that $D_i$ does not intersect any bundle from $\Alloc \setminus A_i$. Then, we have that $D_i \subseteq A_i$, and therefore $R_j = 1$ for all $j \in \agents$. In this case we can set $v_{j,g}$ to be an arbitrary value for all $g \in A_j$, e.g. $v_{j,g} = 1$.
Since Mechanism~\ref{mechanism:NOM+PO+EF1} throws away all goods that have zero value for all agents \alex{this is just saying ``$A_i$ couldn't be smaller'', so it still goes through for submodular}, we have that $A_i = D_i$, and therefore, by definition, the output of Mechanism~\ref{mechanism:NOM+PO+EF1} is precisely $\Alloc$. %\alex{not quite. need to worry about $A_i$ including goods with $v_{i,g} = 0$. These goods, by construction, are not wanted by anyone, but they should somehow end up exactly at $i$'s bundle, which is not what case $\rm{I}$ does (or could do). We should probably adjust the mechanism so that these are just thrown away (currently they go to agent $1$)}

%. In this case, we define $v_j$, the valuation function of agent $j \in [n] \setminus \{i\}$ to be such that $v_{j,g} = 1$ for all goods $g \in B_j$ and $v_{j,g} = 0$ otherwise. Given this, the set of goods desired by agent $j$ is $D_j = B_j$. Since the bundles $\{B_j\}_{j \neq i}$ are pairwise-disjoint, the subsets $\{D_j\}_{j \neq i}$ are pairwise-disjoint as well. Additionally, since $D_i$ does not intersect any bundle from $B_1, B_2, \ldots B_{i-1}, B_{i+1}, \ldots, B_n$, all the subsets $\{D_j\}^n_{j=1}$ are pairwise disjoint. Therefore, Mechanism \ref{mechanism:NOM+PO+EF1} on input $(v_i, v_{-i})$ will output the allocation $(D_1, \ldots, \widehat{D_i}, \ldots, D_n)$. Note that for each agent $j \in [n] \setminus \{i\}$ we have $D_j = B_j$ and by definition, the set $\widehat{D_i} = [m] \setminus \cup_{j\neq i} D_j = [m] \setminus \cup_{j\neq i} B_j = B_i$. Thus, given the reported valuations are $(v_i, v_{-i})$ the mechanism $\widehat{M}$ returns allocation $(B_1, B_2, \ldots, B_n)$.


The second case is that $D_i$ intersects exactly one bundle from $\Alloc \setminus A_i$. Let $j \in (\agents \setminus \{i\})$ be the (unique) agent such that $A_j \cap D_i \neq \emptyset$. Additionally, assume that $i<j$; an almost identical argument works if $i > j$. 
For each agent $k \in \agents \setminus \{i,j\}$, we define $v_{k,g} = 1$ if good $g \in A_k$ and $v_{k,g} = 0$ otherwise. The valuations of agent $j$ are as follows
\[ 
v_{j,g} = \begin{cases} 
      2  v_{i,g} & g \in A_j \cap D_i \alex{update so that the condition is satisfied}\\
      1 & g \in A_j \setminus D_i \\
      0 & otherwise 
   \end{cases}
\]
Note that, the set of desired goods $D_k = A_k$ for all agents $k \in (\agents \setminus \{i\})$, and $\widehat{D}_i = A_i$.
This construction also satisfies that the bundles $\{D_k\}_{k \in \agents \setminus \{i\}}$ are pairwise disjoint, and the bundle $D_i$ only intersects $D_j = A_j$. Therefore, $R_i = R_j = 1$ and $R_k = 0$ for every other agent $k$. Therefore, Mechanism~\ref{mechanism:NOM+PO+EF1}, given valuations $(\values_i, \values_{-i})$, considers $\emph{Case \rm{III}}$ (Lines \ref{case3-begin}-\ref{case3-tie-breaking:end}) to compute the output allocation. In $\emph{Case \rm{III}}$, the mechanism first checks whether $\sum_{g \in D_i \cap D_j} v_{i,g} < \sum_{g \in D_i \cap D_j} v_{j,g}$ holds, which is true for our construction since $v_{j,g} = 2 v_{i,g}$ for $g$ in $A_j \cap D_i = D_j \cap D_i$. Afterwards, the mechanism checks if the allocation $(D_1, \ldots, \widehat{D}_i, \ldots, D_j, \ldots, D_n)$ is $\EFone$ (Line \ref{case3-subcase1-if}). Since this allocation is $\Alloc$ (and $\Alloc \in \EFone(i,\values_i)$), $i$ has an envy of at most one item. Moreover, all other agents are envy-free, since their allocation is precisely all the goods they value. Therefore, Mechanism~\ref{mechanism:NOM+PO+EF1} will indeed output $\Alloc$.

%Indeed the allocation $(D_1, \ldots, \widehat{D}_i, \ldots, D_j, \ldots, D_n)$ -- which is same as the allocation $\mathcal{B} = (B_1, B_2, \ldots, B_n)$ -- is $\EFone$ because agent $i$ doesn't every any other agent (recall that the allocation $\mathcal{B} \in \EFone(i,v_i)$) and every other agent $k \in [n] \setminus \{i\}$ is allocated all the goods they desire, $B_k = D_k$. Thus, the allocation $(D_1, \ldots, \widehat{D}_i, \ldots, D_j, \ldots, D_n)$ (i.e., $(B_1, B_2, \ldots, B_n)$) is $\EFone$, and Mechanism \ref{mechanism:NOM+PO+EF1} outputs this allocation given the input profile $(v_i, v_{-i})$ (Line \ref{case3-subcase1-return}).

The third and final case is that $D_i$ intersects more than one bundle from $\Alloc \setminus A_i$. Here, the valuation vector of each agent $j \in \agents \setminus \{i\}$ is such that $v_{j,g} = 1$ for $g \in A_j$ and $v_{j,g} = 0$ otherwise. By construction, the set of desired goods $D_j = A_j$ for each agent $j \in \agents \setminus \{i\}$, and $\widehat{D}_i = A_i$. Therefore, $D_i$ intersecting more than one bundle from $\Alloc \setminus A_i$, is equivalent to $D_i$ intersecting more than one of the $D_j$ subsets, $j \neq i$, and therefore $R_j = 0$ for all $j \in \agents \setminus \{i\}$. Thus, given the valuation profile $(\values_i, \values_{-i})$, Mechanism~\ref{mechanism:NOM+PO+EF1} considers $\emph{Case \rm{II}}$ (Lines \ref{case2-begin}-\ref{case2-end}), where it will first check whether the allocation $(D_1, D_2, \ldots, \widehat{D}_i, \ldots, D_n)$ is $\EFone$.
This allocation is precisely $\Alloc$, so agent $i$ has an envy of at most one item by definition, and all other agents have no envy at all. Therefore, Mechanism~\ref{mechanism:NOM+PO+EF1} outputs $\Alloc$.

This concludes the proof of Lemma~\ref{lemma:every-EF1-realized}.
\end{proof}


Lemma~\ref{lemma:every-EF1-realized} establishes that all allocations in $\EFone(i,\values_i)$ are possible. Therefore, the problem of whether Mechanism~\ref{mechanism:NOM+PO+EF1} is obviously manipulable (partially) reduces to whether some set $\EFone(i,\values'_i)$ has a better worst-case outcome than $\EFone(i,\values_i)$, with respect to the valuation vector $\values_i$. The following notation will be useful. Given any set of allocations $S \subseteq \Pi_n(\items)$, an agent $i \in \agents$ and a valuation vector $\values$ define 
\[\ell(i,\values, S) = \min_{\Alloc \in S} \ \values(A_i).\]



\begin{lemma}
\label{lemma:least-valued-EF1}
For any pair of valuations $\values,\values' \in \mathbb{R}^m_{\geq 0}$ \alex{update for submodular} and any agent $i \in \agents$, the following inequality holds
\[\ell(i,\values, \EFone(i,\values)) \geq \ell(i,\values, \EFone(i,\values')).\]
\end{lemma}
\begin{proof}
Let $\Alloc = (A_1, A_2, \ldots, A_n) \in \EFone(i,\values)$ be an allocation such $\values(A_i) = \ell(i,\values, \EFone(i,\values))$, i.e. $\Alloc$ is the worst-case outcome for agent $i$ when her valuation vector is $\values$. If $\Alloc \in \EFone(i,\values')$, the lemma immediately follows, since the allocation $\Alloc'$ that minimizes $\values(A'_i)$ over all allocations in $\EFone(i,\values')$ could only be smaller than $\values(A_i)$. Therefore, assume without loss of generality that $\Alloc \notin \EFone(i,\values')$. 

We will construct an allocation $\Alloc'$ with the following properties: $(i)$ $\values(A'_i) \leq \values(A_i)$, and $(ii)$ $\Alloc' \in \EFone(i,\values')$. These two properties together imply the desired inequality, since
$\ell(i,v,\EFone(i,\values)) = \values(A_i) \geq^{\text{by $(i)$}} \values(A'_i) \geq^{\text{by $(ii)$}} \ell(i,\values,\EFone(i,\values'))$.


Let $S^* \subseteq \agents \setminus \{i\}$ be the subset of agents with non-empty bundles in $\Alloc$, i.e., $S^* \coloneqq \{j \in \agents \setminus \{i\} \ | \ A_j \neq \emptyset \}$. Define agent $j^* \coloneqq \argmax_{k \in S^*} \min_{g \in A_k} \values'(A_k \setminus \{g\})$, to be the agent in $S^*$ whose allocation ``up to one item'' has maximum value with respect to $\values'$, and let $g^* = \argmax_{g \in A_{j^*}} \values'(g)$ \alex{update for submodular} be the favorite good with respect to $\values'$ that $j^*$ has. Given these definitions, $\Alloc'$ is defined as follows. $A'_i = A_{j^*} \setminus \{g^*\}$, $A'_{j^*} = A_i \cup \{g^*\}$, and for all agents $k \in \agents \setminus \{i,j^*\}$ we have $A'_k = A_k$. It remains to show that $\Alloc'$ satisfies $(i)$ and $(ii)$.

Towards proving $(i)$ we have %that $\values(A'_i) = \values(A_{j^*} \setminus \{g^*\})$ by
\begin{align}
 \values(A'_i) & = \values(A_{j^*} \setminus \{g^*\}) \tag{by the definition of $A'_i$}\\
 & \leq \values(A_i). \tag{$\Alloc \in \EFone(i,\values)$}
\end{align}

Towards proving $(ii)$, note that $\agents \setminus \{i\}$ can be written as the union of three disjoint sets $S_1$, $S_2$ and $S_3$, where $S_1 = \agents \setminus (S^* \cup \{i\})$, $S_2 = (S^* \setminus \{j^*\})$, and  $S_3 = \{j^*\}$. We will show that in allocation $\Alloc'$ agent $i$ with valuation vector $\values'$, does not envy, up to one item, any of the agents in $S_1$, $S_2$, or $S_3$; this establishes that $\Alloc' \in \EFone(i,\values')$.
First, for every agent $k \in S_1$ we have that $A'_k = A_k = \emptyset$, by the definition of $S^*$, so agent $i$ cannot envy any such agent.
Second, given the definition of agent $j^*$, we know that for each agent $k$ in $S_2 = S^* \setminus \{j^*\}$, we have
\begin{align*}
\min_{g \in A'_k} \values'(A'_k \setminus \{g\}) & = \min_{g \in A_k} \values'(A_k \setminus \{g\}) \tag{$A'_k = A_k$ for all agents except $i$ and $j^*$}\\
& \leq \min_{g \in A_{j^*}} \values'(A_{j^*} \setminus \{g\}) \tag{by the definition of $j^*$} \\
& \leq \values'(A_{j^*} \setminus \{g^*\}) \tag{$g^* \in A_{j^*}$}\\
& = \values'(A'_i). \tag{$A'_i = A_{j^*} \setminus \{g^*\}$}
\end{align*}
That is, agent $i$ with valuation $\values'$ does not envy, up to one item, any agent in $S_2$.

Third, recall that $\Alloc \notin \EFone(i,\values')$. Therefore, by the definition of agent $j^*$ and good $g^*$, it holds that $\values'(A_i) < \values'(A_{j^*} \setminus \{g^*\})$. Therefore,
\begin{align*}
    \values'(A'_i) & = \values'(A_j \setminus \{g^*\}) \tag{$A'_i = A_j \setminus \{g^*\}$} \\
    & > \values'(A_i) \tag{$\Alloc \notin \EFone(i,\values')$} \\
    & = \values'(A_i \cup \{g^*\} \setminus \{g^*\}) \\
    & = \values'(A'_{j^*} \setminus \{g^*\}) \tag{$A'_{j^*} = A_i \cup \{g^*\}$}.
\end{align*}
That is, agent $i$ with valuation $\values'$ does not envy, up to one item, any agent in $S_3 = \{ j^* \}$. 

This establishes that the allocation $\Alloc' \in \EFone(i,v')$ and concludes the proof.
\end{proof}

Now we are ready to prove the main result of this section, Theorem \ref{theorem:NOM+PO+EF1}.

\begin{proof}[Proof of Theorem \ref{theorem:NOM+PO+EF1}]
From Lemma \ref{lemma:PO+EF1} we know that Mechanism~\ref{mechanism:NOM+PO+EF1} always outputs allocations that are EF1 and Pareto efficient. It remains to show that Mechanism~\ref{mechanism:NOM+PO+EF1} is NOM. We first show that agents cannot improve their worst-case utilities by misreporting.

Let $i \in \agents$ be an agent whose true valuation is $\values_i$ and let her misreport be $\bids'_i$. By Lemma~\ref{lemma:every-EF1-realized}, for every reported valuation vector $\values$ of agent $i$, 
and for every allocation $\Alloc \in \EFone(i,\values)$, there exists a valuation profile $\values_{-i}$ such that $\Alloc$ is the output of Mechanism~\ref{mechanism:NOM+PO+EF1}.
On the other hand, Mechanism~\ref{mechanism:NOM+PO+EF1} always outputs allocations that are (1) Pareto efficient; therefore an agent is never allocated an item she has zero value for (and items that have zero value for all agents are thrown away), and (2) envy free up to one item. That is, every output allocation of Mechanism~\ref{mechanism:NOM+PO+EF1} is in $\EFone(i,\values)$.
Therefore, if agent $i$ reports $\values_i$ (respectively $\bids'_i$), then the set of all possible allocations of Mechanism~\ref{mechanism:NOM+PO+EF1} is exactly $\EFone(i,\values_i)$ (respectively $\EFone(i,\bids'_i)$). Therefore, for the worst-case utility of agent $i$ we have

\begin{align*}
    \min\limits_{\values_{-i}} \sum_{j \in \items} v_{i,j} \cdot x_{i,j}(\values_i, \values_{-i}) & = \min\limits_{ \Alloc \in \EFone(i,\values_i)} \values_i(A_i)\\
    & = \ell(i, \values_i, \EFone(i,\values_i)) \tag{by definition} \\
    & \geq \ell(i, \values_i, \EFone(i, \bids'_i)) \tag{Lemma \ref{lemma:least-valued-EF1}}\\
    & = \min\limits_{\values_{-i}} \sum_{j \in \items} v_{i,j} \cdot x_{i,j}(\bids'_i, \values_{-i}).
\end{align*}

This establishes Inequality~\ref{inequality:NOM-worst-case} from the definition of NOM. To conclude the proof, it remains to show that the best-case utility of an agent is also not improved by misreporting. Note that the best case for agent $i \in \agents$ occurs when all other agents \alex{need to add: are additive} report a zero value for all the goods, i.e. $D_j = \emptyset$ for all $j \in \agents \setminus \{i\}$. Hence the sets $\{D_k\}_{k \in [n]}$ are pairwise-disjoint, and Mechanism~\ref{mechanism:NOM+PO+EF1} (via \emph{Case \rm{I}}) allocates the entirety of $D_i$ to agent $i$, which is impossible to improve upon.
\end{proof}

%Given that the mechanism $\widehat{M}$ outputs $\PO + \EFone$ allocations, if the above defined property holds, the following corollary follows.
%
%\begin{corollary}
%The worst case utility for an agent $i$ (as per her true valuation $v^t_i$), if she report her valuation to be $v_i$ is exactly $l(i,v^t_i, \EFone(i,v_i))$.
%\end{corollary}
%Note that, the mechanism $\widehat{M}$ yields $\PO$ allocations, therefore for each agent, her best-case utility under truthful reporting cannot be improved. Given this, the following lemma follows
%
%\begin{lemma}
%If for each agent $i \in [n]$ and every valuation $v_i \in \mathbb{R}^m_{\geq 0}$, the following inequality is true
%\begin{align*}
%l(i,v^t_i, \EFone(i,v^t_i)) \geq l(i,v^t_i, \EFone(i,v_i)),
%\end{align*}
%then the mechanism $\widehat{M}$, which outputs $\PO + \EFone$ allocations, is $\NOM$.
%\end{lemma}


\subsection{Ex-ante EF + Ex-post fPO + Ex-post EF1 + NOM}

In the previous section we established the existence of a deterministic NOM mechanism that outputs ex-post fPO + EF1 allocations. Here we make a short remark that it is not possible to improve upon this result by adding ex-ante fairness guarantees. Specifically, there does not exist a randomized mechanism that is NOM in expectation and outputs ex-post fPO + EF1 allocations that are additionally ex-ante EF. This follows directly from the following impossiblity result proved in \cite{freeman2020best}.

\begin{theorem}[\cite{freeman2020best}]
There exists instances with additive valuation where there is no randomized allocation that is simultaneously ex-post fPO + EF1 and ex-ante EF.
\end{theorem}


==> everything_fix.tex <==
As stated in Section~\ref{sec: intro}, for additive valuations, maximizing the Nash social welfare results in allocations that are fair in addition to being economically efficient ~\cite{caragiannis2019unreasonable}. However, as established in Theorem~\ref{thm: MNW impossibility}, mechanisms that output MNW allocations are obviously manipulable for any number of agents having additive valuations.

In this section we state our main results, which show that there are deterministic $\NOM$ mechanisms that are $(i)$ fair and efficient for additive valuations, $(ii)$ fair and approximately efficient for subadditive valuations and $(iii)$ fair for the general class of monotone valuations. All these results are established by showing a black-box reduction from the problem of designing $\EFone$ and $\NOM$ mechanisms to the problem of designing algorithms that output $\EFone$ allocations. Additionally, this black-box reduction approximately preserves Pareto efficiency guarantees. 

%This result has a number of applications. For example, for the class of additive valuations, we get an $\EFone$, fractionally Pareto efficient and $\NOM$ mechanism, by using in our black-box reduction an algorithm of~\citet{garg2021fair} that returns fPO and EF1 allocations.
The following theorem formally states our main result.


\begin{theorem}\label{theorem:NOM+PO+EF1}
There exists a black-box reduction from the problem of designing a not obviously manipulable and $\EFone$ mechanism for monotone valuations, to designing an algorithm that computes $\EFone$ allocations for monotone valuations. Additionally, the reduction approximately preserves Pareto efficiency guarantees.

Specifically, given an algorithm $\mathcal{M}^*$ that computes $\EFone$ allocations for monotone valuations, we can construct a deterministic not obviously manipulable mechanism that outputs $\EFone$ allocations by using Mechanism \ref{mechanism:NOM+PO+EF1}. Moreover, if $\mathcal{M}^*$ is $\alpha$-Pareto efficient (resp. $\alpha$-fractionally Pareto efficient) then Mechanism~\ref{mechanism:NOM+PO+EF1} always outputs a $\min\{ \alpha, 1 - \epsilon \}$ - Pareto efficient (resp. $\min\{ \alpha, 1 - \epsilon \}$ - fractionally Pareto efficient) allocation, for any $\epsilon > 0$. For the class of additive valuations, $\epsilon = 0$.
\end{theorem}

We establish the above theorem by showing that Mechanism~\ref{mechanism:NOM+PO+EF1}, given black-box access to an $\EFone$ algorithm $\mathcal{M}^*$, always outputs an $\EFone$ allocation (Lemma~\ref{lemma:mech is EF1}) and is additionally not obviously manipulable (Theorem~\ref{thm: EF1 implies NOM}). Furthermore, if $\mathcal{M}^*$ is $\alpha$-Pareto efficient, then Mechanism~\ref{mechanism:NOM+PO+EF1} outputs an (almost) $\alpha$-Pareto efficient allocation (Lemma~\ref{lemma:mech is PO}).

Before we proceed to the applications of Theorem~\ref{theorem:NOM+PO+EF1} and its proof, we briefly comment on the (perhaps counter-intuitive) approximation guarantee for Pareto efficiency. In certain inputs, our reduction attempts to construct an allocation where all agents but one get their the maximum possible utility (i.e., their value for $\items$); if this allocation is also $\EFone$ it is the output of the reduction. For additive agents it is possible to ensure that the last agent gets as much utility as possible (subject to everyone else getting maximum utility) in a computationally efficient way, resulting in a Pareto efficient final allocation. However, for valuation functions beyond additive, it is a computationally challenging task to ensure that some agent gets her maximum possible utility in a way that another agent gets as much utility as possible. We therefore settle for a possibly suboptimal (but still $\EFone$) allocation for the last agent. Now, an allocation where one agent can improve their utility without hurting anyone else is clearly not Pareto efficient. But, at the same time, if one agent gets their maximum possible utility, the corresponding allocation is by definition $(1-\epsilon)$-approximately Pareto efficient, for all $\epsilon > 0$, since any improvement on this agent is impossible. 

%to do this step in a Pareto efficient way, i.e. to ensure that there is no way to improve the utility of an agent without hurting another agent; therefore there is no loss in the efficiency guarantee \paritosh{what is 'this step' in the begining of this line, I  don't understand.}. However,  it is a challenging task to ensure that some agent gets her maximum possible utility in a way that another agent gets as much utility as possible \paritosh{okay, I get that this is challenging. But how does this related to the previous sentence or the next sentence? This seems like an independent comment, the relationship of this comment with approximate Pareto efficiency guarantee is not described.}. An allocation where one agent can improve their utility without hurting anyone else is clearly not Pareto efficient, but at the same time, if one agent gets their maximum possible utility (i.e. their value for $\items$), the corresponding allocation is by definition $(1-\epsilon)$-approximately Pareto efficient, for all $\epsilon > 0$, since any improvement on this agent is impossible. 
%We note that considering a stronger notion of approximate efficiency that demands a point-wise approximation (i.e. a definition of the form ``an allocation $\Alloc$ is $\alpha$-approximately Pareto efficient if there is no allocation $\Alloc'$ such that no agent $i$ can improve their utility by a factor of $\frac{1}{\alpha}$, while 
%See  for a discussion on why this is the right notion of approximate Pareto efficiency. \alex{todo: we basically need to say (somewhere) that the stronger version is ridiculous. E.g. it would imply that various mechanisms provide no guarantees}

%\cite{cole2013mechanism}


\paragraph{Applying the main result}

By combining Theorem~\ref{theorem:NOM+PO+EF1} with known algorithmic results, we can get a number of interesting applications.


For the case of additive agents,~\citet{garg2021fair} gave a pseudo-polynomial time algorithm that computes fractionally Pareto efficient and $\EFone$ allocations. Combining with Theorem~\ref{theorem:NOM+PO+EF1} we get the following result.

\begin{application}\label{application: additive}(via ~\citet{garg2021fair}).
For agents with additive valuations, there exists a fractionally Pareto efficient, $\EFone$, and $\NOM$ mechanism, that runs in pseudo-polynomial time.
\end{application}

%We note that for additive agents applying the ``best of both worlds'' result of~\cite{aziz2020simultaneously} does not give any additional guarantees
%\begin{application}\label{application: matroid rank}(via~\citet{benabbou2021finding}).
%For agents with matroid rank valuations,\footnote{A valuation function $v$ is matroid rank if it's monotone submodular with binary marginals, i.e. (1) $v(S) \leq v(T)$, for $S \subseteq T$, (2) $v(S \cup \{ g \} ) - v(S) \geq v(T \cup \{g\} - V(T)$, for $S \subseteq T$ and $g \notin T$, and (3) $v(S \cup \{ g \} ) - v(S) \in \{ 0 , 1\}$ for all $S \subseteq M$ and $g \in \items$.} there exists a $(1-\epsilon)$-Pareto efficient (for any $\epsilon > 0$), $\EFone$, and $\NOM$ mechanism, that runs in polynomial time.
%\end{application} \paritosh{This is subsumed by the result of Babaioff et al.} \paritosh{Any thoughts? The known result about MRFs are strictly stronger in every aspect: current best is fPO + EFX (even Lorenz domination) + Group strategyproof.}

Next, for agents with subadditive valuation functions,~\citet{chaudhury2021fair} give an algorithm for finding an $\EFone$ allocation that approximates the Nash welfare objective within a factor of $O(n)$ (and therefore gives an $O(n)$ factor approximation for Pareto efficiency).

\begin{application}\label{application: subadditive}
(via~\citet{chaudhury2021fair}).
For agents with subadditive valuation functions, there exists an $\EFone$, $O(n)$-approximately Pareto efficient and $\NOM$ mechanism, that runs in polynomial time, in the value query model.
\end{application}

Finally,~\citet{lipton2003playing} give an algorithm (envy-cycle elimination) for finding an $\EFone$ allocation for monotone valuation functions.

\begin{application}\label{application: monotone}
(via ~\citet{lipton2003playing}).
For agents with monotone valuation functions, there exists an $\EFone$ and $\NOM$ mechanism, that runs in polynomial time, in the value query model.
\end{application}

%\paritosh{A red flag: currently none of our proofs \emph{use} subadditivity. If a reviewer wonders why our reduction only works for subadditive valuations and not generally (since subadditivity is nowhere used), there is no explanation/answer for this in the writeup.}
%\alex{if the main result gets updated to ``monotone'', we should add the subadditive result as a third application.}

%We briefly note that there is an algorithm by~\cite{chaudhury2021fair}, for agents with subadditive valuation functions, that outputs $\EFone$ allocations and approximates the Nash welfare objective within a factor of $O(n)$ (and therefore gives an $O(n)$ factor approximation for Pareto efficiency). Plugging in this algorithm also gives a NOM and $\EFone$ mechanism for subadditive valuations that additionally achieves an $O(n)$ approximation of Pareto efficiency.

%, but the Pareto efficiency guarantee, $O(n)$ approximate Pareto, is the same as in Application~\ref{application: subadditive}. \paritosh{Application 2 doesn't have any efficiency guarantees, and I am not sure whether EF1 by itself provides $\Theta(n)$ Pareto efficiency guarantee --- math doesn't seem to go through.} \alex{you're right. let's change application 2, and mention that lipton et al wouldn't work}


%\paritosh{1. If we are not mentioning efficiency guarantess, we can use envy-cycle elimination [Lipton et al.]. 2. We should add that the result of CGM'21 holds for value oracles.}
%\alex{what is the significance of value oracles?}
%\paritosh{Valuations functions beyond additive valuation required exponential space to explicitly write down, and therefore computational efficiency is argued in terms of query complexity, under appropriate query model. To quote Babaioff et al. "We assume for this purpose that each MRF fi has a succinct representation (of size polynomial in the number m of items) such that given this representation, for every S one may compute fi(S) {\bf (answer value queries)} in time polynomial in m." Additionally, It is known that the result of CGM'21 can be improved upon using the stronger demand queries, but is tight for value queries! So these approximation guarantees are highly dependent on the query model and we should specify it.}

% \paritosh{if it is randomized then our result won't hold right? Our result only establishes } \alex{I think ex-post EF1 suffices, no?} \paritosh{If $\mathcal{M}^*$ is randomized, then we should be showing that our reduction produces a NOM in expectation mechanism, the definition of which asks us to compare expected worst-case utility, where the expectation is taken over random coins used by the mechanism. Since, $\mathcal{M}^*$ is a blackbox, we don't have any info. about the coin tosses done by $\mathcal{M}^*$, and therefore coin-tosses done by our Mechanism 1. So, I think we can't comment on the expected worst-case.}

\subsection{The Reduction}
Our reduction, Mechanism~\ref{mechanism:NOM+PO+EF1}, takes as input reported valuations $\bids = (\bids_1, \dots, \bids_n)$, and black-box access to a deterministic algorithm $\mathcal{M}^*$ \footnote{Algorithm $\mathcal{M}^*$ could possibly be computationally inefficient.}. %$\mathcal{M}^*$ is an arbitrary (not necessarily computationally efficient) algorithm which, given access to agents' valuation functions computes an integral $\EFone$ allocation $\Alloc$. 
Our reduction requires the algorithm $\mathcal{M}^*$ to always output integral EF1 allocations for every possible input valuation functions.

As stated previously, our reduction works even when the valuation functions are monotone. Since, arbitrary monotone functions cannot be specified explicitly, we assume that our mechanism can access the reported valuation functions via value queries, i.e., Mechanism \ref{mechanism:NOM+PO+EF1}, has access to the value oracles corresponding to the reported valuation of each agent. Note that, value oracles are not needed when valuations functions are additive (since they can be specified explicitly using $m$ values), therefore, we can equivalently assume that for additive valuations, Mechanism $1$ receives as an input, the bids $b_{i,j}$ for every $i \in \agents$ and $j \in \items$. %Additionally, the algorithm $\mathcal{M}^*$ is such that it can be executed given value oracles corresponding to the valuation functions. %However, when valuation functions are subadditive, the reported valuations of each agent has to be specified implicitly Mechanism~\ref{mechanism:NOM+PO+EF1} only uses value queries to the reported valuations. %, plus any type of queries needed by $\mathcal{M}^*$.

%\floatname{mechanism}{Mechanism}
\begin{algorithm}[ht]
\caption{Black-box reduction}
\label{mechanism:NOM+PO+EF1}
\hspace*{\algorithmicindent}\textbf{Input:} Value oracles of the reported (monotone) valuation functions of agents $\bids$. Black-box access to an \hspace*{\algorithmicindent} algorithm $\mathcal{M}^*$. \\
\hspace*{\algorithmicindent}\textbf{Output:} A partial integral allocation $\Alloc = (A_1, \ldots, A_n)$ 
%Pseudo code
  \begin{algorithmic}[1]
  		%Initialization
  		\STATE \textbf{Set} $D_i \gets \{ g \in \items \ | \ \bids_i( \{ g \} ) > 0 \}$. \alex{update}
  		\STATE \textbf{Set} $\widehat{D}_i \gets \left( \items \setminus \cup_{j\neq i} D_j \right) \cap D_i$ for each $i \in \agents$.
		\STATE \textbf{Set} $R_i \gets 1$ if subsets $\{D_j\}^n_{j=1} \setminus \{D_i\}$ are pairwise disjoint; $0$ otherwise.
		\tikzmark{top1}
  		\IF{the subsets $\{D_j\}_{j=1}^n$ are pairwise disjoint 	}
  			\STATE $\Alloc^* \gets (D_1, \ldots, D_n)$
  		\tikzmark{bottom1}
  		\tikzmark{top2}
  		\ELSIF{$\exists i \in \agents$ such that $R_i = 1$ and $R_j = 0$ for every $j \in \agents \setminus \{i\}$} \label{case2-begin}
  			\IF{the allocation $(D_1, D_2, \ldots, \widehat{D}_i, \ldots, D_n)$ is $\EFone$}
  				\STATE $\Alloc^* \gets (D_1, D_2, \ldots, \widehat{D}_i, \ldots, D_n)$ \label{case2-return1}
  			\ELSE
  				\STATE $\Alloc^* \gets \mathcal{M}^*(\bids_1, \bids_2, \ldots, \bids_n)$
  			\ENDIF \label{case2-end}
  		\tikzmark{bottom2}
  		\tikzmark{top3}
  		\ELSIF{$\exists i,j \in \agents$ such that $i<j$ and $R_i = R_j = 1$, and $R_k =0$ for $k \in [n] \setminus \{i,j\}$}~~~~~~\tikzmark{right} \label{case3-begin}
  			\IF{$\bids_i(D_i \cap D_j) < \bids_j(D_i \cap D_j)$} \label{case3-tie-breaking:begin}
				\IF{$(D_1, \ldots, \widehat{D}_i, \ldots, D_j, \ldots, D_n)$ is $\EFone$} \label{case3-subcase1-if} 
					\STATE $\Alloc^* \gets (D_1, \ldots, \widehat{D}_i, \ldots, D_j, \ldots, D_n)$ \label{case3-subcase1-return}
				\ELSE
					\STATE $\Alloc^* \gets \mathcal{M}^*(\bids_1, \bids_2, \ldots, \bids_n)$
				\ENDIF  \label{case3-subcase1:end}		
  			\ELSE \label{case3-subcase2:begin}
				\IF{$(D_1, \ldots, D_i, \ldots, \widehat{D}_j, \ldots, D_n)$ is $\EFone$} 
					\STATE $\Alloc^* \gets (D_1, \ldots, D_i, \ldots, \widehat{D}_j, \ldots, D_n)$
				\ELSE
					\STATE $\Alloc^* \gets \mathcal{M}^*(\bids_1, \bids_2, \ldots, \bids_n)$ 
				\ENDIF 
  			\ENDIF \label{case3-tie-breaking:end}
  			\tikzmark{bottom3}
  		\tikzmark{top4}
  		\ELSE
  			\STATE $\Alloc^* \gets \mathcal{M}^*(\bids_1, \bids_2, \ldots, \bids_n)$
  		\ENDIF
  		\tikzmark{bottom4}
  		%\STATE For all $i \in \agents$, iteratively remove goods $g \in \Alloc^*_i$ such that $\bids_i( \Alloc^*_i \setminus \{ g \} ) = \bids_i( \Alloc^*_i )$. \label{code:removal}
  		\STATE \textbf{return} $\Alloc^*$
		\end{algorithmic}
		\AddNote{top1}{bottom1}{right}{\emph{Case $\rm{I}$}}
		\AddNote{top2}{bottom2}{right}{\emph{Case $\rm{II}$}}
		\AddNote{top3}{bottom3}{right}{\emph{Case $\rm{III}$}}
		\AddNote{top4}{bottom4}{right}{\emph{Case $\rm{IV}$}}
\end{algorithm}




Let $D_i$ be a minimal set of goods such that $\values_i(D_i) = \values_i(\items)$. Specifically, we set $D_i = \items$, and proceed to consider items in lexicographical order, repeatedly removing an item $g \in D_i$ if $\values_i(D_i \setminus \{ g \}) = \values_i(D_i)$, until no such good exists. For additive agents, this is just the set of items that $i$ has a strictly positive value for. Notice that this operation yields a unique set $D_i$ for each agent.
%the set of goods that have strictly positive marginal value, over the empty set, i.e. $D_i \coloneqq \{ g \in \items \ | \ \bids_i( \{ g \} ) > 0 \}$. For additive agents, this is just the set of items that $i$ has a strictly positive value for. Notice that $\values_i(D_i) = \values_i(\items)$, by subadditivity. \alex{update}
Let $\widehat{D}_i \coloneqq \items \setminus \cup_{j\neq i} D_j$ be the set of items remaining after removing all goods desired by agents other than $i$. Finally, let $R_i$, for each agent $i \in \agents$, be the indicator for the event that the subsets $( \{D_j\}_{j \in \agents}) \setminus \{D_i\}$ are pairwise disjoint, i.e. $R_i = 1$ iff $( \{D_j\}_{j \in \agents}) \setminus \{D_i\}$ are pairwise disjoint, and $R_i = 0$ otherwise. Note that the $R_i$s can be easily computed in polynomial time, since the sets $D_i$s can be computed efficiently by using value queries. Mechanism~\ref{mechanism:NOM+PO+EF1} sequentially considers four cases based on the sets $\{D_j\}^n_{j=1}$ and the values $\{R_j\}^n_{j=1}$, to find a temporary assignment $\Alloc^*$.

\begin{description}
\item[\emph{Case \rm{I}}:] The sets $\{D_j\}^n_{j=1}$ are pairwise disjoint (equivalently, $R_i = 1$ for all $i \in \agents$). In this case, the temporary assignment allocates the bundle $D_j$ to agent $j$ for each agent $j \in \agents$.
\item[\emph{Case \rm{II}}:] $R_i = 1$ for exactly one agent $i \in \agents$. This can occur if $D_i$ intersects with two or more $D_j$s (and these are the only intersections). In this case, if allocating the bundle $\widehat{D}_i$ to agent $i$, and the bundle $D_j$ to each agent $j \in \agents$, $j \neq i$ is $\EFone$, then the temporary assignment is this allocation (note that, by definition, this is a feasible allocation). Otherwise, if this allocation is not $\EFone$, the temporary assignment is the allocation of the black-box algorithm $\mathcal{M}^*$ for the given valuation profile.
\item[\emph{Case \rm{III}}:] There are exactly two agents $i,j \in \agents$ such that $R_i = R_j = 1$. Note that the only way this is possible is if $D_i$, $D_j$ intersect each other and any other pair of subsets $D_k, D_l$ where $\{k,l\} \neq \{i,j\}$, are disjoint. In this case, Mechanism~\ref{mechanism:NOM+PO+EF1} considers whether the set of goods $D_i \cap D_j$ are valued more by agent $i$ or agent $j$; each of these two subcases are similar to \emph{Case \rm{II}}, see Lines \ref{case3-tie-breaking:begin}-\ref{case3-tie-breaking:end}.
\item[\emph{Case \rm{IV}}:] None of the previous cases holds (equivalently, $R_i = 0$ for all $i \in \agents$). In this case, the temporary assignment is simply the allocation of the black-box algorithm $\mathcal{M}^*$ for the given valuation profile.
\end{description}

The last step of Mechanism~\ref{mechanism:NOM+PO+EF1} is to make the the temporary allocation of each agent $i$ \emph{clean}, i.e. remove items from her bundle, as long as that doesn't change her value for her bundle. Formally, we iteratively remove a good $g \in A^*_i$ if $\bids_i(A^*_i) = \bids_i(A^*_i \setminus \{g \})$; ties can be broken in an arbitrary manner. This step is necessary for one of our technical lemmas (specifically, we need to argue about the set of all allocations that are possible outputs of our mechanism), but note that it does not affect efficiency nor envy-freeness up to one item (i.e. if the allocation satisfied any of these notions before this step, it continues to do so).



%In \emph{Case \rm{I}}, the set of goods desired by agent $\{D_j\}^n_{j=1}$ are pairwise disjoint, and the mechanism allocates the bundle $D_j$ to agent $j$ for each agent $j \in \agents$. 
%Otherwise, in \emph{Case \rm{II}}, there is a single agent $i \in \agents$ such that $R_i = 1$. Note that, the conditions corresponding to these cases are checked sequentially, as a consequence, in cases other than \emph{Case \rm{I}}, the sets $\{D_j\}^n_{j=1}$ are not pairwise disjoint. Thus, in \emph{Case \rm{II}} the subsets $\{D_j\}^n_{j=1}$ are not pairwise disjoint and there is one agent $i \in \agents$ such that $R_i = 1$, i.e., the subsets $\{D_j\}^n_{j=1} \setminus \{D_i\}$ are pairwise disjoint. In this case, if the allocation $(D_1, D_2, \ldots, \widehat{D}_i, \ldots, D_n)$ is $\EFone$ then the mechanism $\widehat{M}$ returns it, otherwise it return the allocation that mechanism $M$ (the blackbox mechanism for $\PO+\EFone$) would return for the given valuations. 
%In \emph{Case \rm{III}}, there are exactly two agents $i,j \in \agents$ having $R_i = R_j = 1$, and the subsets $\{D_j\}^n_{j=1}$ are not pairwise disjoint. Note that, this can happen only if the subsets $D_i$, $D_j$ intersect each other and any other pair of subsets $D_k, D_l$ where $\{k,l\} \neq \{i,j\}$ are disjoint. Here, the mechanism considers two subcases based on whether the set of goods $D_i \cap D_j$ are valued more by agent $i$ or agent $j$; each of these two subcases are similar to \emph{Case \rm{II}}, see Lines \ref{case3-tie-breaking:begin}-\ref{case3-tie-breaking:end}. Finally, in \emph{Case \rm{IV}}, the mechanism simply returns the allocation that the blackbox mechanism $M$ would output for the given valuation profile.


\paragraph{Establishing the main result}

Towards establishing our main result, Theorem \ref{theorem:NOM+PO+EF1}, we begin by proving the following supporting lemmas. We start by showing that Mechanism~\ref{mechanism:NOM+PO+EF1} preserves the efficiency properties of $\mathcal{M}^*$. 
We will then proceed to show that Mechanism~\ref{mechanism:NOM+PO+EF1} also preserves EF1 if $\mathcal{M}^*$ is EF1, and, in fact, Mechanism~\ref{mechanism:NOM+PO+EF1} is also NOM when $\mathcal{M}^*$ is EF1.

\begin{lemma}
\label{lemma:mech is PO}
For agents with monotone valuation functions, if $\mathcal{M}^*$ is $\alpha$-Pareto efficient (resp. $\alpha$-fractionally Pareto efficient) then Mechanism~\ref{mechanism:NOM+PO+EF1} always outputs a $\min\{ \alpha, 1 - \epsilon \}$ - Pareto efficient (resp. $\min\{ \alpha, 1 - \epsilon \}$ - fractionally Pareto efficient) allocation, for any $\epsilon > 0$. For additive agents, $\epsilon = 0$.
\end{lemma}

\begin{proof}
First, notice that Line~\ref{code:removal} does not affect the utility of any agent $i$ for her own bundle. %, i.e. this step does not affect the outcome in utility space. 
Therefore if the allocation before this step was $\beta$-PO (respectively $\beta$-fPO) then after Line~\ref{code:removal} these efficiency guarantees will continue to hold. Considering all possible cases for Mechanism~\ref{mechanism:NOM+PO+EF1}, if all agents $j \in \agents$ receive the bundle $D_j$ (as in case \rm{I}), the allocation is fractionally Pareto efficient. If all agents $j$ receive the bundle $D_j$, with the exception of a single agent $i$ that receives $\widehat{D}_i$, then all agents except $i$ have the maximum possible utility.
If agents are additive, it is impossible to improve the utility of $i$ without hurting some other agent $j$; therefore, this allocation is fractionally Pareto efficient for additive agents. More generally for monotone agents, it is infeasible to give an agent $j \neq i$ utility strictly greater than their current utility, i.e. the current allocation is $(1-\epsilon)$ fractionally Pareto efficient, for every $\epsilon > 0$. This allocation is considered in cases \rm{II} and \rm{III} (if $\mathcal{M}^*$ is not called), and it is the output of Mechanism~\ref{mechanism:NOM+PO+EF1} if it is also $\EFone$. Finally, in the remaining cases (if the aforementioned allocation is not $\EFone$, or we are in case \rm{IV}) Mechanism~\ref{mechanism:NOM+PO+EF1} returns the same allocation as the black-box algorithm $\mathcal{M}^*$ would return, which is $\alpha$-PO (respectively $\alpha$-fPO) by definition.
\end{proof}



\begin{lemma}
\label{lemma:mech is EF1}
If $\mathcal{M}^*$ is $\EFone$ then Mechanism~\ref{mechanism:NOM+PO+EF1} always outputs a clean and $\EFone$ allocation.
\end{lemma}

\begin{proof}
Line~\ref{code:removal} does not affect the utility of any agent for her own bundle, and since valuations are monotone, could only decrease her utility for the bundle of a different agent. Therefore if the allocation before this step was $\EFone$, it remains $\EFone$ afterwards. This step also ensures that allocation is clean. Next, considering all possible cases, we first have that if every agent $j \in \agents$ receives the bundle $D_j$ (as in case \rm{I}), the allocation is envy-free, and therefore $\EFone$. In cases \rm{II} and \rm{III}, Mechanism~\ref{mechanism:NOM+PO+EF1} checks whether an allocation is $\EFone$ before outputting it, or calls $\mathcal{M}^*$. In case \rm{IV} $\mathcal{M}^*$ is called. Finally, if $\mathcal{M}^*$ is called, then the output allocation is $\EFone$ by definition. 
\end{proof}



The next lemma characterizes the set of allocations that Mechanism~\ref{mechanism:NOM+PO+EF1} could possibly return given the reported valuation of a particular agent. 
Specifically, we will show that every clean, non-wasteful and $\EFone$ allocation, that is consistent with the reported valuation, is possible. Before stating the lemma, we define some useful notation.
For any agent $i \in \agents$ and monotone valuation function $\values_i$, let $\EFone(i,\values_i)$ be the set of allocations $\Alloc = (A_1, \ldots, A_n)$ that are clean, non-wasteful and envy-free up to one item with respect to agent $i$ when her valuation function is $\values_i$, i.e., 
%Let $\Pi^*_n(\items)$ be the set of partial allocations of $\items$, i.e. ordered subpartitions of $\items$ into $\agents$ bundles.
$\EFone(i,\values_i) = \{ \Alloc \in \Pi_n(\items) \ | \forall j \in \agents \text{ with } A_j \neq \emptyset, \values_i(A_i) \geq \values_i(A_j \setminus \{g\}) \text{ for some }g \in A_j, \text{ and }  A_i \subseteq D_i, \text{ and } \forall g \in D_i \setminus A_i, \exists j \in \agents \text{ such that } g \in A_j \}$.
%\paritosh{If we require each bundle to be 'clean', then the resultant allocation may not even be a partition -- $\Alloc \in \Pi_n(\items)$ is incorrect.}  \alex{fixed. double-check} \paritosh{Included the definition of Pi^*_n(\items) in the prelims and changes it to Pi_n(\items). Prelims now has definition of both partial and complete allocations.}


\begin{lemma}
\label{lemma:every-EF1-realized}
Given any agent $i \in \agents$ and monotone valuation function $\values_i$, for every allocation $\Alloc \in \EFone(i,\values_i)$ there exists a set of valuations $\values_{-i}$ such that Mechanism~\ref{mechanism:NOM+PO+EF1} on input  $(\values_i, \values_{-i})$ outputs allocation $\Alloc$.
\end{lemma}

%\paritosh{Continue Cleanup from here}

\begin{proof}
Given the valuation vector $\values_i$ and an allocation $\Alloc = (A_1, A_2, \dots, A_n) \in \EFone(i,\values_i)$ we will construct valuations for the other agents, $\values_{-i}$, such that Mechanism~\ref{mechanism:NOM+PO+EF1} outputs $\Alloc$ on input  $(\values_i, \values_{-i})$.  The valuation function $\values_j$ of each agent $j \neq i$ will be additive. Specifically, the constructed valuation of each agent $j \in (\agents \setminus \{i\})$ will be such that $v_{j,g} = 0$ for all $g \notin A_j$, and $v_{j,g} > 0$ for each good $g \in A_j$ (the precise value of $v_{j,g}$ will depend on how $D_i$ intersects with $A_j$). That is, for each agent $j \in (\agents \setminus \{i\})$, $D_j = A_j$. Therefore, by construction, the subsets $\{D_j\}^n_{j=1} \setminus \{D_i\}$ are pairwise disjoint, and therefore $R_i = 1$ (so, we are never in case $\rm{IV}$ of Mechanism~\ref{mechanism:NOM+PO+EF1}).
In the rest of the proof, we consider the three exhaustive cases, based on how many sets from $\Alloc_{-i} = (A_1, \dots, A_{i-1}, A_{i+1}, \dots)$ %\setminus A_i$ \paritosh{incorrect notation: subtracting a set from a n-tuple!} 
the set $D_i$ intersects.

The first case is that $D_i$ does not intersect any bundle from $\Alloc_{-i}$. In this case we can set $v_{j,g}$ to be an arbitrary value for all $g \in A_j$, e.g. $v_{j,g} = 1$, for all agents $j \neq i$. We have that $R_j = 1$ for all $j \in \agents$, and therefore Mechanism~\ref{mechanism:NOM+PO+EF1} considers $\emph{Case \rm{I}}$, and it allocates the set $D_j$ to every agent $j$.
For $j \neq i$, it is immediate that $D_j = A_j$. By the definition of $\EFone(i,\values_i)$, $A_i \subseteq D_i$ and all goods in $D_i$ not allocated to $i$ must be allocated to some other agent. However, since no other agent's allocation overlaps with $D_i$, it must be that $A_i = D_i$ as well. Therefore, the output of Mechanism~\ref{mechanism:NOM+PO+EF1} is precisely $\Alloc$. 

The second case is that $D_i$ intersects exactly one bundle from $\Alloc_{-i}$. Let $j^* \in (\agents \setminus \{i\})$ be the (unique) agent such that $A_{j^*} \cap D_i \neq \emptyset$. Additionally, assume that $i<j^*$; an almost identical argument works if $i > j^*$. 
For each agent $k \in \agents \setminus \{i,j^*\}$, we define $v_{k,g} = 1$ if good $g \in A_k$ and $v_{k,g} = 0$ otherwise. The valuations of agent $j^*$ are as follows
\[ 
v_{j^*,g} = \begin{cases} 
      2  \values_i (D_i \cap D_{j^*}) & g \in A_{j^*} \cap D_i \\
      1 & g \in A_{j^*} \setminus D_i \\
      0 & otherwise 
   \end{cases}
\]
Note that, the set of desired goods $D_k = A_k$ for all agents $k \in (\agents \setminus \{i\})$. Also, $\widehat{D}_i = \left( \items \setminus \cup_{j\neq i} D_j \right) \cap D_i =\left( \items \setminus \cup_{j\neq i} A_j \right) \cap D_i$ is precisely the subset of $D_i$ not allocated to agents other than $i$; since every item in $D_i$ not allocated to $i$ must be allocated to another agent (by the definition of $\EFone(i,\values_i)$), we have that $\widehat{D}_i = A_i$.
This construction also satisfies that the bundles $\{D_k\}_{k \in \agents \setminus \{i\}}$ are pairwise disjoint, and the bundle $D_i$ only intersects $D_{j^*} = A_{j^*}$. Therefore, $R_i = R_{j^*} = 1$ and $R_k = 0$ for every other agent $k$. Therefore, Mechanism~\ref{mechanism:NOM+PO+EF1}, given valuations $(\values_i, \values_{-i})$, considers $\emph{Case \rm{III}}$ (Lines \ref{case3-begin}-\ref{case3-tie-breaking:end}) to compute the final allocation. In $\emph{Case \rm{III}}$, the mechanism first checks whether $\values_i (D_i \cap D_{j^*}) < \values_j (D_i \cap D_{j^*})$ holds, which is true for our construction since $v_{j^*,g} = 2 \values_i (D_i \cap D_{j^*})$ for all $g$ in $A_{j^*} \cap D_i = D_{j^*} \cap D_i$. Afterwards, the mechanism checks if the allocation $(D_1, \ldots, \widehat{D}_i, \ldots, D_{j^*}, \ldots, D_n)$ is $\EFone$ (Line \ref{case3-subcase1-if}). Since this allocation is $\Alloc$ (and $\Alloc \in \EFone(i,\values_i)$), $i$ has an envy of at most one item. Moreover, all other agents are envy-free, since their allocation is precisely all the goods they value. Therefore, Mechanism~\ref{mechanism:NOM+PO+EF1} will indeed output $\Alloc$. 



The third and final case is that $D_i$ intersects more than one bundle from $\Alloc_{-i}$. Here, the valuation vector of every agent $j \in \agents \setminus \{i\}$ is such that $v_{j,g} = 1$ for $g \in A_j$ and $v_{j,g} = 0$ otherwise. By construction, the set of desired goods $D_j = A_j$ for every agent $j \in \agents \setminus \{i\}$, and, similarly to the previous case, $\widehat{D}_i = \left( \items \setminus \cup_{j\neq i} A_j \right) \cap D_i = A_i$. Therefore, $D_i$ intersecting more than one bundle from $\Alloc_{-i}$, is equivalent to $D_i$ intersecting more than one of the $D_j$ subsets, $j \neq i$, and therefore $R_j = 0$ for all $j \in \agents \setminus \{i\}$. Thus, given the valuation profile $(\values_i, \values_{-i})$, Mechanism~\ref{mechanism:NOM+PO+EF1} considers $\emph{Case \rm{II}}$ (Lines \ref{case2-begin}-\ref{case2-end}), where it first checks whether the allocation $(D_1, D_2, \ldots, \widehat{D}_i, \ldots, D_n)$ is $\EFone$. This allocation is precisely $\Alloc$, so agent $i$ has an envy of at most one item by definition, and all other agents have no envy at all. Therefore, Mechanism~\ref{mechanism:NOM+PO+EF1} outputs $\Alloc$.
This concludes the proof of Lemma~\ref{lemma:every-EF1-realized}.
\end{proof}


Lemma~\ref{lemma:every-EF1-realized} establishes that all allocations in $\EFone(i,\values_i)$ are possible. Therefore, the problem of whether Mechanism~\ref{mechanism:NOM+PO+EF1} is obviously manipulable (partially) reduces to whether some set $\EFone(i,\values'_i)$ has a better worst-case outcome than $\EFone(i,\values_i)$, with respect to the valuation vector $\values_i$. The following notation will be useful. Given any set of allocations $S \subseteq \Pi_n(\items)$, an agent $i \in \agents$ and a valuation vector $\values$ define 
\[\ell(i,\values, S) = \min_{\Alloc \in S} \ \values(A_i).\]


%\paritosh{add a remark (maybe at the end) that subadditivity is never used in the proof, it works for general monotone valuations}
\begin{lemma}
\label{lemma:least-valued-EF1}
For any pair of monotone valuation functions $\values,\values'$ and any agent $i \in \agents$, the following inequality holds
\[\ell(i,\values, \EFone(i,\values)) \geq \ell(i,\values, \EFone(i,\values')).\]
\end{lemma}
\begin{proof}
Let $\Alloc = (A_1, A_2, \ldots, A_n) \in \EFone(i,\values)$ be an allocation such $\values(A_i) = \ell(i,\values, \EFone(i,\values))$, i.e. $\Alloc$ is the worst-case outcome for agent $i$ when her valuation vector is $\values$. If $\Alloc \in \EFone(i,\values')$, the lemma immediately follows, since the allocation $\Alloc'$ that minimizes $\values(A'_i)$ over all allocations in $\EFone(i,\values')$ could only be smaller than $\values(A_i)$. Therefore, assume without loss of generality that $\Alloc \notin \EFone(i,\values')$. We will construct an allocation $\Alloc'$ with the following properties: $(i)$ $\values(A'_i) \leq \values(A_i)$, and $(ii)$ $\Alloc' \in \EFone(i,\values')$. These two properties together imply the desired inequality, since
$\ell(i,\values,\EFone(i,\values)) = \values(A_i) \geq \values(A'_i) \geq \ell(i,\values,\EFone(i,\values'))$, where the first inequality follows from $(i)$ and the second inequality follows from $(ii)$.


Let $S^* \subseteq \agents \setminus \{i\}$ be the subset of agents with non-empty bundles in $\Alloc$, i.e., $S^* \coloneqq \{j \in \agents \setminus \{i\} \ | \ A_j \neq \emptyset \}$. Define agent $j^* \coloneqq \argmax_{k \in S^*} \min_{g \in A_k} \values'(A_k \setminus \{g\})$, to be the agent in $S^*$ whose allocation ``up to one item'' has maximum value with respect to $\values'$, and let $g^* = \argmin_{g \in A_{j^*}} \values'(A_{j^*} \setminus \{g\})$ be the favorite good with respect to $\values'$ that $j^*$ has. Given these definitions, $\Alloc'$ is defined as follows. $A'_i = A_{j^*} \setminus \{g^*\}$, $A'_{j^*} = A_i \cup \{g^*\}$, and for all agents $k \in \agents \setminus \{i,j^*\}$ we have $A'_k = A_k$. It remains to show that $\Alloc'$ satisfies $(i)$ and $(ii)$.

Towards proving $(i)$ we have $\values(A'_i) = \values(A_{j^*} \setminus \{g^*\}) \leq \values(A_i)$, where the last inequality follows from the fact that $\Alloc \in \EFone(i,\values)$.

Towards proving $(ii)$, note that $\agents \setminus \{i\}$ can be written as the union of three disjoint sets $S_1$, $S_2$ and $S_3$, where $S_1 = \agents \setminus (S^* \cup \{i\})$, $S_2 = (S^* \setminus \{j^*\})$, and  $S_3 = \{j^*\}$. We will show that in allocation $\Alloc'$ agent $i$ with valuation vector $\values'$, does not envy, up to one item, any of the agents in $S_1$, $S_2$, or $S_3$; this establishes that $\Alloc' \in \EFone(i,\values')$.
First, for every agent $k \in S_1$ we have that $A'_k = A_k = \emptyset$, by the definition of $S^*$, so agent $i$ cannot envy any such agent.
Second, given the definition of agent $j^*$, we know that for each agent $k$ in $S_2 = S^* \setminus \{j^*\}$, we have
\begin{align*}
\min_{g \in A'_k} \values'(A'_k \setminus \{g\}) & = \min_{g \in A_k} \values'(A_k \setminus \{g\}) \tag{$A'_k = A_k$ for all agents except $i$ and $j^*$}\\
& \leq \min_{g \in A_{j^*}} \values'(A_{j^*} \setminus \{g\}) \tag{by the definition of $j^*$} \\
& \leq \values'(A_{j^*} \setminus \{g^*\}) \tag{$g^* \in A_{j^*}$}\\
& = \values'(A'_i). \tag{$A'_i = A_{j^*} \setminus \{g^*\}$}
\end{align*}

Therefore, agent $i$ with valuation $\values'$ does not envy up to one item (and, in fact, up to any item) any agent in $S_2$.

Third, recall that $\Alloc \notin \EFone(i,\values')$. By definition, agent $j^*$ has the bundle that $\values'$ likes the most ``up to one item'', and $g^*$ is that most valuable (in terms of marginal value) item in $j^*$'s bundle, so $\values'(A_i) < \values'(A_{j^*} \setminus \{g^*\})$. Therefore, we have
\begin{align*}
    \values'(A'_i) & = \values'(A_j \setminus \{g^*\}) \tag{$A'_i = A_j \setminus \{g^*\}$} \\
    & > \values'(A_i) \tag{$\Alloc \notin \EFone(i,\values')$} \\
    & = \values'(A_i \cup \{g^*\} \setminus \{g^*\}) \\
    & = \values'(A'_{j^*} \setminus \{g^*\}) \tag{$A'_{j^*} = A_i \cup \{g^*\}$}.
\end{align*}
That is, agent $i$ with valuation $\values'$ does not envy, up to one item, any agent in $S_3 = \{ j^* \}$. 

This establishes that $\Alloc' \in \EFone(i,v')$ and concludes the proof.
\end{proof}

Given the previous lemmas, we can show our main theorem with respect to not obviously manipulability.

\begin{theorem}\label{thm: EF1 implies NOM}
If agents' valuation functions are monotone and $\mathcal{M}^*$ is $\EFone$, then Mechanism~\ref{mechanism:NOM+PO+EF1} is not obviously manipulable.
\end{theorem}

\begin{proof}
We first show that agents cannot improve their worst-case utilities by misreporting.

Let $i \in \agents$ be an agent whose true valuation is $\values_i$ and let her misreport be $\bids_i$. By Lemma~\ref{lemma:every-EF1-realized}, for every reported valuation vector $\bids$ of agent $i$, 
and for every allocation $\Alloc \in \EFone(i,\bids)$, there exists a valuation profile $\values_{-i}$ such that $\Alloc$ is the output of Mechanism~\ref{mechanism:NOM+PO+EF1}.
On the other hand, Mechanism~\ref{mechanism:NOM+PO+EF1} always outputs allocations $\Alloc$ that are (1) clean (by Line~\ref{code:addition}), and (2) envy free up to one item (Lemma~\ref{lemma:mech is EF1}). That is, every output allocation of Mechanism~\ref{mechanism:NOM+PO+EF1} is in $\EFone(i,\bids)$.
Therefore, if agent $i$ reports $\values_i$ (respectively $\bids_i$), then the set of all possible allocations of Mechanism~\ref{mechanism:NOM+PO+EF1} is exactly $\EFone(i,\values_i)$ (respectively $\EFone(i,\bids_i)$).
Overloading notation, let $A^*_i(\values_i, \values_{-i})$ be the allocation of agent $i$ in Mechanism~\ref{mechanism:NOM+PO+EF1}, on input $(\values_i, \values_{-i})$.
For the worst-case utility of agent $i$ we have
\begin{align*}
    \min\limits_{\values_{-i}} \values_i( A^*_i(\values_i, \values_{-i})  )& = \min\limits_{ \Alloc \in \EFone(i,\values_i)} \values_i(A_i)\\
    & = \ell(i, \values_i, \EFone(i,\values_i)) \tag{by definition} \\
    & \geq \ell(i, \values_i, \EFone(i, \bids_i)) \tag{Lemma \ref{lemma:least-valued-EF1}}\\
    & = \min\limits_{\values_{-i}} \values_i( A^*_i(\bids_i, \values_{-i})  ).
\end{align*}

This establishes Inequality~\ref{inequality:NOM-worst-case} from the definition of NOM. To conclude the proof, it remains to show that the best-case utility of an agent is also not improved by misreporting. Note that the best case for agent $i \in \agents$ occurs when all other agents have no value for the items, i.e. $D_j = \emptyset$ for all $j \in \agents \setminus \{i\}$. Hence the sets $\{D_k\}_{k \in [n]}$ are pairwise-disjoint, and Mechanism~\ref{mechanism:NOM+PO+EF1} (via \emph{Case \rm{I}}) allocates the entirety of $D_i$ to agent $i$, which is impossible to improve upon.
\end{proof}



%Now we are ready to prove the main result of this section, Theorem %\ref{theorem:NOM+PO+EF1}.

%\begin{proof}[Proof of Theorem \ref{theorem:NOM+PO+EF1}]

%\end{proof}

%Given that the mechanism $\widehat{M}$ outputs $\PO + \EFone$ allocations, if the above defined property holds, the following corollary follows.
%
%\begin{corollary}
%The worst case utility for an agent $i$ (as per her true valuation $v^t_i$), if she report her valuation to be $v_i$ is exactly $l(i,v^t_i, \EFone(i,v_i))$.
%\end{corollary}
%Note that, the mechanism $\widehat{M}$ yields $\PO$ allocations, therefore for each agent, her best-case utility under truthful reporting cannot be improved. Given this, the following lemma follows
%
%\begin{lemma}
%If for each agent $i \in [n]$ and every valuation $v_i \in \mathbb{R}^m_{\geq 0}$, the following inequality is true
%\begin{align*}
%l(i,v^t_i, \EFone(i,v^t_i)) \geq l(i,v^t_i, \EFone(i,v_i)),
%\end{align*}
%then the mechanism $\widehat{M}$, which outputs $\PO + \EFone$ allocations, is $\NOM$.
%\end{lemma}


\subsection{Ex-ante EF, Ex-post fPO, Ex-post EF1 and NOM}

In the previous section we established (Application~\ref{application: additive}) the existence of a deterministic NOM mechanism that outputs ex-post fPO and EF1 allocations for additive agents. Here we make a short remark that it is not possible to improve upon this result by adding ex-ante fairness guarantees. Specifically, there does not exist a randomized mechanism that is NOM in expectation and outputs ex-post fPO and EF1 allocations, that is additionally ex-ante envy-free. This follows directly from the following impossibility result of~\citet{freeman2020best}.

\begin{theorem}[\cite{freeman2020best}]
There exists instances with additive valuation where there is no randomized allocation that is simultaneously ex-post fPO and $\EFone$, and ex-ante envy-free.
\end{theorem}


==> everything_subadditive.tex <==
As stated in Section~\ref{sec: intro}, for additive valuations, maximizing the Nash social welfare results in allocations that are fair in addition to being economically efficient ~\cite{caragiannis2019unreasonable}. However, as established in Theorem~\ref{thm: MNW impossibility}, mechanisms that output MNW allocations are obviously manipulable for any number of agents having additive valuations.

In this section we state our main results, which show that there are deterministic $\NOM$ mechanisms that are $(i)$ fair and efficient for additive valuations, $(ii)$ fair and approximately efficient for subadditive valuations and $(iii)$ fair for the general class of monotone valuations. All these results are established by showing a black-box reduction from the problem of designing $\EFone$ and $\NOM$ mechanisms to the problem of designing algorithms that output $\EFone$ allocations. Additionally, this black-box reduction approximately preserves Pareto efficiency guarantees. 

%This result has a number of applications. For example, for the class of additive valuations, we get an $\EFone$, fractionally Pareto efficient and $\NOM$ mechanism, by using in our black-box reduction an algorithm of~\citet{garg2021fair} that returns fPO and EF1 allocations.
The following theorem formally states our main result.


\begin{theorem}\label{theorem:NOM+PO+EF1}
There exists a black-box reduction from the problem of designing a not obviously manipulable and $\EFone$ mechanism for monotone valuations, to designing an algorithm that computes $\EFone$ allocations for monotone valuations. Additionally, the reduction approximately preserves Pareto efficiency guarantees.

Specifically, given an algorithm $\mathcal{M}^*$ that computes $\EFone$ allocations for monotone valuations, we can construct a deterministic not obviously manipulable mechanism that outputs $\EFone$ allocations by using Mechanism \ref{mechanism:NOM+PO+EF1}. Moreover, if $\mathcal{M}^*$ is $\alpha$-Pareto efficient (resp. $\alpha$-fractionally Pareto efficient) then Mechanism~\ref{mechanism:NOM+PO+EF1} always outputs a $\min\{ \alpha, 1 - \epsilon \}$ - Pareto efficient (resp. $\min\{ \alpha, 1 - \epsilon \}$ - fractionally Pareto efficient) allocation, for any $\epsilon > 0$. For the class of additive valuations, $\epsilon = 0$.
\end{theorem}

We establish the above theorem by showing that Mechanism~\ref{mechanism:NOM+PO+EF1}, given black-box access to an $\EFone$ algorithm $\mathcal{M}^*$, always outputs an $\EFone$ allocation (Lemma~\ref{lemma:mech is EF1}) and is additionally not obviously manipulable (Theorem~\ref{thm: EF1 implies NOM}). Furthermore, if $\mathcal{M}^*$ is $\alpha$-Pareto efficient, then Mechanism~\ref{mechanism:NOM+PO+EF1} outputs an (almost) $\alpha$-Pareto efficient allocation (Lemma~\ref{lemma:mech is PO}).

Before we proceed to the applications of Theorem~\ref{theorem:NOM+PO+EF1} and its proof, we briefly comment on the (perhaps counter-intuitive) approximation guarantee for Pareto efficiency. In certain inputs, our reduction attempts to construct an allocation where all agents but one get their the maximum possible utility (i.e., their value for $\items$); if this allocation is also $\EFone$ it is the output of the reduction. For additive agents it is possible to ensure that the last agent gets as much utility as possible (subject to everyone else getting maximum utility) in a computationally efficient way, resulting in a Pareto efficient final allocation. However, for valuation functions beyond additive, it is a computationally challenging task to ensure that some agent gets her maximum possible utility in a way that another agent gets as much utility as possible. We therefore settle for a possibly suboptimal (but still $\EFone$) allocation for the last agent. Now, an allocation where one agent can improve their utility without hurting anyone else is clearly not Pareto efficient. But, at the same time, if one agent gets their maximum possible utility, the corresponding allocation is by definition $(1-\epsilon)$-approximately Pareto efficient, for all $\epsilon > 0$, since any improvement on this agent is impossible. 

%to do this step in a Pareto efficient way, i.e. to ensure that there is no way to improve the utility of an agent without hurting another agent; therefore there is no loss in the efficiency guarantee \paritosh{what is 'this step' in the begining of this line, I  don't understand.}. However,  it is a challenging task to ensure that some agent gets her maximum possible utility in a way that another agent gets as much utility as possible \paritosh{okay, I get that this is challenging. But how does this related to the previous sentence or the next sentence? This seems like an independent comment, the relationship of this comment with approximate Pareto efficiency guarantee is not described.}. An allocation where one agent can improve their utility without hurting anyone else is clearly not Pareto efficient, but at the same time, if one agent gets their maximum possible utility (i.e. their value for $\items$), the corresponding allocation is by definition $(1-\epsilon)$-approximately Pareto efficient, for all $\epsilon > 0$, since any improvement on this agent is impossible. 
%We note that considering a stronger notion of approximate efficiency that demands a point-wise approximation (i.e. a definition of the form ``an allocation $\Alloc$ is $\alpha$-approximately Pareto efficient if there is no allocation $\Alloc'$ such that no agent $i$ can improve their utility by a factor of $\frac{1}{\alpha}$, while 
%See  for a discussion on why this is the right notion of approximate Pareto efficiency. \alex{todo: we basically need to say (somewhere) that the stronger version is ridiculous. E.g. it would imply that various mechanisms provide no guarantees}

%\cite{cole2013mechanism}


\paragraph{Applying the main result}

By combining Theorem~\ref{theorem:NOM+PO+EF1} with known algorithmic results, we can get a number of interesting applications.


For the case of additive agents,~\citet{garg2021fair} gave a pseudo-polynomial time algorithm that computes fractionally Pareto efficient and $\EFone$ allocations. Combining with Theorem~\ref{theorem:NOM+PO+EF1} we get the following result.

\begin{application}\label{application: additive}(via ~\citet{garg2021fair}).
For agents with additive valuations, there exists a fractionally Pareto efficient, $\EFone$, and $\NOM$ mechanism, that runs in pseudo-polynomial time.
\end{application}

%We note that for additive agents applying the ``best of both worlds'' result of~\cite{aziz2020simultaneously} does not give any additional guarantees
%\begin{application}\label{application: matroid rank}(via~\citet{benabbou2021finding}).
%For agents with matroid rank valuations,\footnote{A valuation function $v$ is matroid rank if it's monotone submodular with binary marginals, i.e. (1) $v(S) \leq v(T)$, for $S \subseteq T$, (2) $v(S \cup \{ g \} ) - v(S) \geq v(T \cup \{g\} - V(T)$, for $S \subseteq T$ and $g \notin T$, and (3) $v(S \cup \{ g \} ) - v(S) \in \{ 0 , 1\}$ for all $S \subseteq M$ and $g \in \items$.} there exists a $(1-\epsilon)$-Pareto efficient (for any $\epsilon > 0$), $\EFone$, and $\NOM$ mechanism, that runs in polynomial time.
%\end{application} \paritosh{This is subsumed by the result of Babaioff et al.} \paritosh{Any thoughts? The known result about MRFs are strictly stronger in every aspect: current best is fPO + EFX (even Lorenz domination) + Group strategyproof.}

Next, for agents with subadditive valuation functions,~\citet{chaudhury2021fair} give an algorithm for finding an $\EFone$ allocation that approximates the Nash welfare objective within a factor of $O(n)$ (and therefore gives an $O(n)$ factor approximation for Pareto efficiency).

\begin{application}\label{application: subadditive}
(via~\citet{chaudhury2021fair}).
For agents with subadditive valuation functions, there exists an $\EFone$, $O(n)$-approximately Pareto efficient and $\NOM$ mechanism, that runs in polynomial time, in the value query model.
\end{application}

Finally,~\citet{lipton2003playing} give an algorithm (envy-cycle elimination) for finding an $\EFone$ allocation for monotone valuation functions.

\begin{application}\label{application: monotone}
(via ~\citet{lipton2003playing}).
For agents with monotone valuation functions, there exists an $\EFone$ and $\NOM$ mechanism, that runs in polynomial time, in the value query model.
\end{application}

%\paritosh{A red flag: currently none of our proofs \emph{use} subadditivity. If a reviewer wonders why our reduction only works for subadditive valuations and not generally (since subadditivity is nowhere used), there is no explanation/answer for this in the writeup.}
%\alex{if the main result gets updated to ``monotone'', we should add the subadditive result as a third application.}

%We briefly note that there is an algorithm by~\cite{chaudhury2021fair}, for agents with subadditive valuation functions, that outputs $\EFone$ allocations and approximates the Nash welfare objective within a factor of $O(n)$ (and therefore gives an $O(n)$ factor approximation for Pareto efficiency). Plugging in this algorithm also gives a NOM and $\EFone$ mechanism for subadditive valuations that additionally achieves an $O(n)$ approximation of Pareto efficiency.

%, but the Pareto efficiency guarantee, $O(n)$ approximate Pareto, is the same as in Application~\ref{application: subadditive}. \paritosh{Application 2 doesn't have any efficiency guarantees, and I am not sure whether EF1 by itself provides $\Theta(n)$ Pareto efficiency guarantee --- math doesn't seem to go through.} \alex{you're right. let's change application 2, and mention that lipton et al wouldn't work}


%\paritosh{1. If we are not mentioning efficiency guarantess, we can use envy-cycle elimination [Lipton et al.]. 2. We should add that the result of CGM'21 holds for value oracles.}
%\alex{what is the significance of value oracles?}
%\paritosh{Valuations functions beyond additive valuation required exponential space to explicitly write down, and therefore computational efficiency is argued in terms of query complexity, under appropriate query model. To quote Babaioff et al. "We assume for this purpose that each MRF fi has a succinct representation (of size polynomial in the number m of items) such that given this representation, for every S one may compute fi(S) {\bf (answer value queries)} in time polynomial in m." Additionally, It is known that the result of CGM'21 can be improved upon using the stronger demand queries, but is tight for value queries! So these approximation guarantees are highly dependent on the query model and we should specify it.}

% \paritosh{if it is randomized then our result won't hold right? Our result only establishes } \alex{I think ex-post EF1 suffices, no?} \paritosh{If $\mathcal{M}^*$ is randomized, then we should be showing that our reduction produces a NOM in expectation mechanism, the definition of which asks us to compare expected worst-case utility, where the expectation is taken over random coins used by the mechanism. Since, $\mathcal{M}^*$ is a blackbox, we don't have any info. about the coin tosses done by $\mathcal{M}^*$, and therefore coin-tosses done by our Mechanism 1. So, I think we can't comment on the expected worst-case.}

\subsection{The Reduction}
Our reduction, Mechanism~\ref{mechanism:NOM+PO+EF1}, takes as input reported valuations $\bids = (\bids_1, \dots, \bids_n)$, and black-box access to a deterministic algorithm $\mathcal{M}^*$ \footnote{Algorithm $\mathcal{M}^*$ could possibly be computationally inefficient.}. %$\mathcal{M}^*$ is an arbitrary (not necessarily computationally efficient) algorithm which, given access to agents' valuation functions computes an integral $\EFone$ allocation $\Alloc$. 
Our reduction requires the algorithm $\mathcal{M}^*$ to always output integral EF1 allocations for every possible input valuation functions.

As stated previously, our reduction works even when the valuation functions are monotone. Since, arbitrary monotone functions cannot be specified explicitly, we assume that our mechanism can access the reported valuation functions via value queries, i.e., Mechanism \ref{mechanism:NOM+PO+EF1}, has access to the value oracles corresponding to the reported valuation of each agent. Note that, value oracles are not needed when valuations functions are additive (since they can be specified explicitly using $m$ values), therefore, we can equivalently assume that for additive valuations, Mechanism $1$ receives as an input, the bids $b_{i,j}$ for every $i \in \agents$ and $j \in \items$. %Additionally, the algorithm $\mathcal{M}^*$ is such that it can be executed given value oracles corresponding to the valuation functions. %However, when valuation functions are subadditive, the reported valuations of each agent has to be specified implicitly Mechanism~\ref{mechanism:NOM+PO+EF1} only uses value queries to the reported valuations. %, plus any type of queries needed by $\mathcal{M}^*$.

%\floatname{mechanism}{Mechanism}
\begin{algorithm}[ht]
\caption{Black-box reduction}
\label{mechanism:NOM+PO+EF1}
\hspace*{\algorithmicindent}\textbf{Input:} Value oracles of the reported (monotone) valuation functions of agents $\bids$. Black-box access to an \hspace*{\algorithmicindent} algorithm $\mathcal{M}^*$. \\
\hspace*{\algorithmicindent}\textbf{Output:} A partial integral allocation $\Alloc = (A_1, \ldots, A_n)$ 
%Pseudo code
  \begin{algorithmic}[1]
  		%Initialization
  		\STATE \textbf{Set} $D_i \gets \{ g \in \items \ | \ \bids_i( \{ g \} ) > 0 \}$. \alex{update}
  		\STATE \textbf{Set} $\widehat{D}_i \gets \items \setminus \cup_{j\neq i} D_j$ for each $i \in \agents$.
		\STATE \textbf{Set} $R_i \gets 1$ if subsets $\{D_j\}^n_{j=1} \setminus \{D_i\}$ are pairwise disjoint; $0$ otherwise.
		\tikzmark{top1}
  		\IF{the subsets $\{D_j\}_{j=1}^n$ are pairwise disjoint 	}
  			\STATE $\Alloc^* \gets (D_1, \ldots, D_n)$
  		\tikzmark{bottom1}
  		\tikzmark{top2}
  		\ELSIF{$\exists i \in \agents$ such that $R_i = 1$ and $R_j = 0$ for every $j \in \agents \setminus \{i\}$} \label{case2-begin}
  			\IF{the allocation $(D_1, D_2, \ldots, \widehat{D}_i, \ldots, D_n)$ is $\EFone$}
  				\STATE $\Alloc^* \gets (D_1, D_2, \ldots, \widehat{D}_i, \ldots, D_n)$ \label{case2-return1}
  			\ELSE
  				\STATE $\Alloc^* \gets \mathcal{M}^*(\bids_1, \bids_2, \ldots, \bids_n)$
  			\ENDIF \label{case2-end}
  		\tikzmark{bottom2}
  		\tikzmark{top3}
  		\ELSIF{$\exists i,j \in \agents$ such that $i<j$ and $R_i = R_j = 1$, and $R_k =0$ for $k \in [n] \setminus \{i,j\}$}~~~~~~\tikzmark{right} \label{case3-begin}
  			\IF{$\bids_i(D_i \cap D_j) < \bids_j(D_i \cap D_j)$} \label{case3-tie-breaking:begin}
				\IF{$(D_1, \ldots, \widehat{D}_i, \ldots, D_j, \ldots, D_n)$ is $\EFone$} \label{case3-subcase1-if} 
					\STATE $\Alloc^* \gets (D_1, \ldots, \widehat{D}_i, \ldots, D_j, \ldots, D_n)$ \label{case3-subcase1-return}
				\ELSE
					\STATE $\Alloc^* \gets \mathcal{M}^*(\bids_1, \bids_2, \ldots, \bids_n)$
				\ENDIF  \label{case3-subcase1:end}		
  			\ELSE \label{case3-subcase2:begin}
				\IF{$(D_1, \ldots, D_i, \ldots, \widehat{D}_j, \ldots, D_n)$ is $\EFone$} 
					\STATE $\Alloc^* \gets (D_1, \ldots, D_i, \ldots, \widehat{D}_j, \ldots, D_n)$
				\ELSE
					\STATE $\Alloc^* \gets \mathcal{M}^*(\bids_1, \bids_2, \ldots, \bids_n)$ 
				\ENDIF 
  			\ENDIF \label{case3-tie-breaking:end}
  			\tikzmark{bottom3}
  		\tikzmark{top4}
  		\ELSE
  			\STATE $\Alloc^* \gets \mathcal{M}^*(\bids_1, \bids_2, \ldots, \bids_n)$
  		\ENDIF
  		\tikzmark{bottom4}
  		\STATE For all $i \in \agents$, iteratively remove goods $g \in \Alloc^*_i$ such that $\bids_i( \Alloc^*_i \setminus \{ g \} ) = \bids_i( \Alloc^*_i )$. \label{code:removal}
  		\STATE \textbf{return} $\Alloc^*$
		\end{algorithmic}
		\AddNote{top1}{bottom1}{right}{\emph{Case $\rm{I}$}}
		\AddNote{top2}{bottom2}{right}{\emph{Case $\rm{II}$}}
		\AddNote{top3}{bottom3}{right}{\emph{Case $\rm{III}$}}
		\AddNote{top4}{bottom4}{right}{\emph{Case $\rm{IV}$}}
\end{algorithm}




Let $D_i$ be a minimal set of goods such that $\values_i(D_i) = \values_i(\items)$. Specifically, we set $D_i = \items$, and proceed to consider items in lexicographical order, repeatedly removing an item $g \in D_i$ if $\values_i(D_i \setminus \{ g \}) = \values_i(D_i)$, until no such good exists. For additive agents, this is just the set of items that $i$ has a strictly positive value for. Notice that this operation yields a unique set $D_i$ for each agent.
%the set of goods that have strictly positive marginal value, over the empty set, i.e. $D_i \coloneqq \{ g \in \items \ | \ \bids_i( \{ g \} ) > 0 \}$. For additive agents, this is just the set of items that $i$ has a strictly positive value for. Notice that $\values_i(D_i) = \values_i(\items)$, by subadditivity. \alex{update}
Let $\widehat{D}_i \coloneqq \items \setminus \cup_{j\neq i} D_j$ be the set of items remaining after removing all goods desired by agents other than $i$. Finally, let $R_i$, for each agent $i \in \agents$, be the indicator for the event that the subsets $( \{D_j\}_{j \in \agents}) \setminus \{D_i\}$ are pairwise disjoint, i.e. $R_i = 1$ iff $( \{D_j\}_{j \in \agents}) \setminus \{D_i\}$ are pairwise disjoint, and $R_i = 0$ otherwise. Note that the $R_i$s can be easily computed in polynomial time, since the sets $D_i$s can be computed efficiently by using value queries. Mechanism~\ref{mechanism:NOM+PO+EF1} sequentially considers four cases based on the sets $\{D_j\}^n_{j=1}$ and the values $\{R_j\}^n_{j=1}$, to find a temporary assignment $\Alloc^*$.

\begin{description}
\item[\emph{Case \rm{I}}:] The sets $\{D_j\}^n_{j=1}$ are pairwise disjoint (equivalently, $R_i = 1$ for all $i \in \agents$). In this case, the temporary assignment allocates the bundle $D_j$ to agent $j$ for each agent $j \in \agents$.
\item[\emph{Case \rm{II}}:] $R_i = 1$ for exactly one agent $i \in \agents$. This can occur if $D_i$ intersects with two or more $D_j$s (and these are the only intersections). In this case, if allocating the bundle $\widehat{D}_i$ to agent $i$, and the bundle $D_j$ to each agent $j \in \agents$, $j \neq i$ is $\EFone$, then the temporary assignment is this allocation (note that, by definition, this is a feasible allocation). Otherwise, if this allocation is not $\EFone$, the temporary assignment is the allocation of the black-box algorithm $\mathcal{M}^*$ for the given valuation profile.
\item[\emph{Case \rm{III}}:] There are exactly two agents $i,j \in \agents$ such that $R_i = R_j = 1$. Note that the only way this is possible is if $D_i$, $D_j$ intersect each other and any other pair of subsets $D_k, D_l$ where $\{k,l\} \neq \{i,j\}$, are disjoint. In this case, Mechanism~\ref{mechanism:NOM+PO+EF1} considers whether the set of goods $D_i \cap D_j$ are valued more by agent $i$ or agent $j$; each of these two subcases are similar to \emph{Case \rm{II}}, see Lines \ref{case3-tie-breaking:begin}-\ref{case3-tie-breaking:end}.
\item[\emph{Case \rm{IV}}:] None of the previous cases holds (equivalently, $R_i = 0$ for all $i \in \agents$). In this case, the temporary assignment is simply the allocation of the black-box algorithm $\mathcal{M}^*$ for the given valuation profile.
\end{description}

The last step of Mechanism~\ref{mechanism:NOM+PO+EF1} is to make the the temporary allocation of each agent $i$ \emph{clean}, i.e. remove items from her bundle, as long as that doesn't change her value for her bundle. Formally, we iteratively remove a good $g \in A^*_i$ if $\bids_i(A^*_i) = \bids_i(A^*_i \setminus \{g \})$; ties can be broken in an arbitrary manner. This step is necessary for one of our technical lemmas (specifically, we need to argue about the set of all allocations that are possible outputs of our mechanism), but note that it does not affect efficiency nor envy-freeness up to one item (i.e. if the allocation satisfied any of these notions before this step, it continues to do so).



%In \emph{Case \rm{I}}, the set of goods desired by agent $\{D_j\}^n_{j=1}$ are pairwise disjoint, and the mechanism allocates the bundle $D_j$ to agent $j$ for each agent $j \in \agents$. 
%Otherwise, in \emph{Case \rm{II}}, there is a single agent $i \in \agents$ such that $R_i = 1$. Note that, the conditions corresponding to these cases are checked sequentially, as a consequence, in cases other than \emph{Case \rm{I}}, the sets $\{D_j\}^n_{j=1}$ are not pairwise disjoint. Thus, in \emph{Case \rm{II}} the subsets $\{D_j\}^n_{j=1}$ are not pairwise disjoint and there is one agent $i \in \agents$ such that $R_i = 1$, i.e., the subsets $\{D_j\}^n_{j=1} \setminus \{D_i\}$ are pairwise disjoint. In this case, if the allocation $(D_1, D_2, \ldots, \widehat{D}_i, \ldots, D_n)$ is $\EFone$ then the mechanism $\widehat{M}$ returns it, otherwise it return the allocation that mechanism $M$ (the blackbox mechanism for $\PO+\EFone$) would return for the given valuations. 
%In \emph{Case \rm{III}}, there are exactly two agents $i,j \in \agents$ having $R_i = R_j = 1$, and the subsets $\{D_j\}^n_{j=1}$ are not pairwise disjoint. Note that, this can happen only if the subsets $D_i$, $D_j$ intersect each other and any other pair of subsets $D_k, D_l$ where $\{k,l\} \neq \{i,j\}$ are disjoint. Here, the mechanism considers two subcases based on whether the set of goods $D_i \cap D_j$ are valued more by agent $i$ or agent $j$; each of these two subcases are similar to \emph{Case \rm{II}}, see Lines \ref{case3-tie-breaking:begin}-\ref{case3-tie-breaking:end}. Finally, in \emph{Case \rm{IV}}, the mechanism simply returns the allocation that the blackbox mechanism $M$ would output for the given valuation profile.


\paragraph{Establishing the main result}

Towards establishing our main result, Theorem \ref{theorem:NOM+PO+EF1}, we begin by proving the following supporting lemmas. We start by showing that Mechanism~\ref{mechanism:NOM+PO+EF1} preserves the efficiency properties of $\mathcal{M}^*$. 
We will then proceed to show that Mechanism~\ref{mechanism:NOM+PO+EF1} also preserves EF1 if $\mathcal{M}^*$ is EF1, and, in fact, Mechanism~\ref{mechanism:NOM+PO+EF1} is also NOM when $\mathcal{M}^*$ is EF1.

\begin{lemma}
\label{lemma:mech is PO}
For agents with monotone valuation functions, if $\mathcal{M}^*$ is $\alpha$-Pareto efficient (resp. $\alpha$-fractionally Pareto efficient) then Mechanism~\ref{mechanism:NOM+PO+EF1} always outputs a $\min\{ \alpha, 1 - \epsilon \}$ - Pareto efficient (resp. $\min\{ \alpha, 1 - \epsilon \}$ - fractionally Pareto efficient) allocation, for any $\epsilon > 0$. For additive agents, $\epsilon = 0$.
\end{lemma}

\begin{proof}
First, notice that Line~\ref{code:removal} does not affect the utility of any agent $i$ for her own bundle. %, i.e. this step does not affect the outcome in utility space. 
Therefore if the allocation before this step was $\beta$-PO (respectively $\beta$-fPO) then after Line~\ref{code:removal} these efficiency guarantees will continue to hold. Considering all possible cases for Mechanism~\ref{mechanism:NOM+PO+EF1}, if all agents $j \in \agents$ receive the bundle $D_j$ (as in case \rm{I}), the allocation is fractionally Pareto efficient. If all agents $j$ receive the bundle $D_j$, with the exception of a single agent $i$ that receives $\widehat{D}_i$, then all agents except $i$ have the maximum possible utility.
If agents are additive, it is impossible to improve the utility of $i$ without hurting some other agent $j$; therefore, this allocation is fractionally Pareto efficient for additive agents. More generally for monotone agents, it is infeasible to give an agent $j \neq i$ utility strictly greater than their current utility, i.e. the current allocation is $(1-\epsilon)$ fractionally Pareto efficient, for every $\epsilon > 0$. This allocation is considered in cases \rm{II} and \rm{III} (if $\mathcal{M}^*$ is not called), and it is the output of Mechanism~\ref{mechanism:NOM+PO+EF1} if it is also $\EFone$. Finally, in the remaining cases (if the aforementioned allocation is not $\EFone$, or we are in case \rm{IV}) Mechanism~\ref{mechanism:NOM+PO+EF1} returns the same allocation as the black-box algorithm $\mathcal{M}^*$ would return, which is $\alpha$-PO (respectively $\alpha$-fPO) by definition.
\end{proof}



\begin{lemma}
\label{lemma:mech is EF1}
If $\mathcal{M}^*$ is $\EFone$ then Mechanism~\ref{mechanism:NOM+PO+EF1} always outputs a clean and $\EFone$ allocation.
\end{lemma}

\begin{proof}
Line~\ref{code:removal} does not affect the utility of any agent for her own bundle, and since valuations are monotone, could only decrease her utility for the bundle of a different agent. Therefore if the allocation before this step was $\EFone$, it remains $\EFone$ afterwards. This step also ensures that allocation is clean. Next, considering all possible cases, we first have that if every agent $j \in \agents$ receives the bundle $D_j$ (as in case \rm{I}), the allocation is envy-free, and therefore $\EFone$. In cases \rm{II} and \rm{III}, Mechanism~\ref{mechanism:NOM+PO+EF1} checks whether an allocation is $\EFone$ before outputting it, or calls $\mathcal{M}^*$. In case \rm{IV} $\mathcal{M}^*$ is called. Finally, if $\mathcal{M}^*$ is called, then the output allocation is $\EFone$ by definition. 
\end{proof}



The next lemma characterizes the set of allocations that Mechanism~\ref{mechanism:NOM+PO+EF1} could possibly return given the reported valuation of a particular agent. 
Specifically, we will show that every clean, non-wasteful and $\EFone$ allocation, that is consistent with the reported valuation, is possible. Before stating the lemma, we define some useful notation.
For any agent $i \in \agents$ and monotone valuation function $\values_i$, let $\EFone(i,\values_i)$ be the set of allocations $\Alloc = (A_1, \ldots, A_n)$ that are clean, non-wasteful and envy-free up to one item with respect to agent $i$ when her valuation function is $\values_i$, i.e., 
%Let $\Pi^*_n(\items)$ be the set of partial allocations of $\items$, i.e. ordered subpartitions of $\items$ into $\agents$ bundles.
$\EFone(i,\values_i) = \{ \Alloc \in \Pi_n(\items) \ | \ \forall g \in A_i ~~ \values_i(A_i \setminus \{ g \} ) < \values_i(A_i), \text{ and } \forall j \in \agents \text{ with } A_j \neq \emptyset, \values_i(A_i) \geq \values_i(A_j \setminus \{g\}) \text{ for some }g \in A_j, \text{ and }  \values_i( A_i \cup \left( \items \setminus \cup_{k \in \agents} A_k \right) ) = \values_i (A_i)  \}$.
%\paritosh{If we require each bundle to be 'clean', then the resultant allocation may not even be a partition -- $\Alloc \in \Pi_n(\items)$ is incorrect.}  \alex{fixed. double-check} \paritosh{Included the definition of Pi^*_n(\items) in the prelims and changes it to Pi_n(\items). Prelims now has definition of both partial and complete allocations.}


\begin{lemma}
\label{lemma:every-EF1-realized}
Given any agent $i \in \agents$ and monotone valuation function $\values_i$, for every allocation $\Alloc \in \EFone(i,\values_i)$ there exists a set of valuations $\values_{-i}$ such that Mechanism~\ref{mechanism:NOM+PO+EF1} on input  $(\values_i, \values_{-i})$ outputs allocation $\Alloc$.
\end{lemma}

%\paritosh{Continue Cleanup from here}

\begin{proof}
Given the valuation vector $\values_i$ and an allocation $\Alloc = (A_1, A_2, \dots, A_n) \in \EFone(i,\values_i)$ we will construct valuations for the other agents, $\values_{-i}$, such that Mechanism~\ref{mechanism:NOM+PO+EF1} outputs $\Alloc$ on input  $(\values_i, \values_{-i})$.  The valuation function $\values_j$ of each agent $j \neq i$ will be additive. Specifically, the constructed valuation of each agent $j \in (\agents \setminus \{i\})$ will be such that $v_{j,g} = 0$ for all $g \notin A_j$, and $v_{j,g} > 0$ for each good $g \in A_j$ (the precise value of $v_{j,g}$ will depend on how $D_i$ intersects with $A_j$). That is, for each agent $j \in (\agents \setminus \{i\})$, $D_j = A_j$. Therefore, by construction, the subsets $\{D_j\}^n_{j=1} \setminus \{D_i\}$ are pairwise disjoint, and therefore $R_i = 1$ (so, we are never in case $\rm{IV}$ of Mechanism~\ref{mechanism:NOM+PO+EF1}). Also, by construction, Line~\ref{code:removal} will not affect any bundle.
In the rest of the proof, we consider the three exhaustive cases, based on how many sets from $\Alloc_{-i} = (A_1, \dots, A_{i-1}, A_{i+1}, \dots)$ %\setminus A_i$ \paritosh{incorrect notation: subtracting a set from a n-tuple!} 
the set $D_i$ intersects.

The first case is that $D_i$ does not intersect any bundle from $\Alloc_{-i}$. Then, we have that $D_i \subseteq A_i$ (since $\Alloc$ is a feasible allocation), and therefore $R_j = 1$ for all $j \in \agents$. In this case we can set $v_{j,g}$ to be an arbitrary value for all $g \in A_j$, e.g. $v_{j,g} = 1$, for all agents $j \neq i$.
Therefore, Mechanism~\ref{mechanism:NOM+PO+EF1} considers $\emph{Case \rm{I}}$, and it allocates the set $D_j$ to every agent $j$. For all $j \neq i$, $D_j = A_j$, by definition. For agent $i$, since $A_i$ is also clean (by Line~\ref{code:removal}), it must also be that $A_i = D_i$. Therefore, the output of Mechanism~\ref{mechanism:NOM+PO+EF1} is precisely $\Alloc$. 

The second case is that $D_i$ intersects exactly one bundle from $\Alloc_{-i}$. Let $j^* \in (\agents \setminus \{i\})$ be the (unique) agent such that $A_{j^*} \cap D_i \neq \emptyset$. Additionally, assume that $i<j^*$; an almost identical argument works if $i > j^*$. 
For each agent $k \in \agents \setminus \{i,j^*\}$, we define $v_{k,g} = 1$ if good $g \in A_k$ and $v_{k,g} = 0$ otherwise. The valuations of agent $j^*$ are as follows
\[ 
v_{j^*,g} = \begin{cases} 
      2  \values_i (D_i \cap D_{j^*}) & g \in A_{j^*} \cap D_i \\
      1 & g \in A_{j^*} \setminus D_i \\
      0 & otherwise 
   \end{cases}
\]
Note that, the set of desired goods $D_k = A_k$ for all agents $k \in (\agents \setminus \{i\})$, and $\widehat{D}_i = A_i$. \alex{this should be $A_i \subseteq \widehat{D}_i$ }\paritosh{right. At least for additive valuations, this checks out --- $A_i$ is cleaned version of $\widehat{D}_i$} This construction also satisfies that the bundles $\{D_k\}_{k \in \agents \setminus \{i\}}$ are pairwise disjoint, and the bundle $D_i$ only intersects $D_{j^*} = A_{j^*}$. Therefore, $R_i = R_{j^*} = 1$ and $R_k = 0$ for every other agent $k$. Therefore, Mechanism~\ref{mechanism:NOM+PO+EF1}, given valuations $(\values_i, \values_{-i})$, considers $\emph{Case \rm{III}}$ (Lines \ref{case3-begin}-\ref{case3-tie-breaking:end}) to compute the final allocation. In $\emph{Case \rm{III}}$, the mechanism first checks whether $\values_i (D_i \cap D_{j^*}) < \values_j (D_i \cap D_{j^*})$ holds, which is true for our construction since $v_{j^*,g} = 2 \values_i (D_i \cap D_{j^*})$ for all $g$ in $A_{j^*} \cap D_i = D_{j^*} \cap D_i$. Afterwards, the mechanism checks if the allocation $(D_1, \ldots, \widehat{D}_i, \ldots, D_{j^*}, \ldots, D_n)$ is $\EFone$ (Line \ref{case3-subcase1-if}). Since this allocation is $\Alloc$ (and $\Alloc \in \EFone(i,\values_i)$), $i$ has an envy of at most one item. Moreover, all other agents are envy-free, since their allocation is precisely all the goods they value. Therefore, Mechanism~\ref{mechanism:NOM+PO+EF1} will indeed output $\Alloc$. \alex{potential issue: algo gives you $\widehat{D}_i$ which is a strict superset of $A_i$. since $A$ is non-wasteful, it must be that $\values_i(\widehat{D}_i)= \values_i(A_i)$, but will the algo ``clean'' $\widehat{D}_i$ to $A_i$?}\paritosh{thinking about a solution for this.}
\alex{maybe we need to re-define EF1(v) to only have complete allocations}
\paritosh{I think then we end up with the problem where $A_i$ has items that aren't in $D_i$, and our reduction is oblivious to such items (it considers only items in $D_i$).}

The third and final case is that $D_i$ intersects more than one bundle from $\Alloc_{-i}$. Here, the valuation vector of every agent $j \in \agents \setminus \{i\}$ is such that $v_{j,g} = 1$ for $g \in A_j$ and $v_{j,g} = 0$ otherwise. By construction, the set of desired goods $D_j = A_j$ for every agent $j \in \agents \setminus \{i\}$, and $\widehat{D}_i = A_i$. Therefore, $D_i$ intersecting more than one bundle from $\Alloc_{-i}$, is equivalent to $D_i$ intersecting more than one of the $D_j$ subsets, $j \neq i$, and therefore $R_j = 0$ for all $j \in \agents \setminus \{i\}$. Thus, given the valuation profile $(\values_i, \values_{-i})$, Mechanism~\ref{mechanism:NOM+PO+EF1} considers $\emph{Case \rm{II}}$ (Lines \ref{case2-begin}-\ref{case2-end}), where it first checks whether the allocation $(D_1, D_2, \ldots, \widehat{D}_i, \ldots, D_n)$ is $\EFone$. This allocation is precisely $\Alloc$, so agent $i$ has an envy of at most one item by definition, and all other agents have no envy at all. Therefore, Mechanism~\ref{mechanism:NOM+PO+EF1} outputs $\Alloc$.
This concludes the proof of Lemma~\ref{lemma:every-EF1-realized}.\alex{same here}
\end{proof}


Lemma~\ref{lemma:every-EF1-realized} establishes that all allocations in $\EFone(i,\values_i)$ are possible. Therefore, the problem of whether Mechanism~\ref{mechanism:NOM+PO+EF1} is obviously manipulable (partially) reduces to whether some set $\EFone(i,\values'_i)$ has a better worst-case outcome than $\EFone(i,\values_i)$, with respect to the valuation vector $\values_i$. The following notation will be useful. Given any set of allocations $S \subseteq \Pi_n(\items)$, an agent $i \in \agents$ and a valuation vector $\values$ define 
\[\ell(i,\values, S) = \min_{\Alloc \in S} \ \values(A_i).\]


%\paritosh{add a remark (maybe at the end) that subadditivity is never used in the proof, it works for general monotone valuations}
\begin{lemma}
\label{lemma:least-valued-EF1}
For any pair of monotone valuation functions $\values,\values'$ and any agent $i \in \agents$, the following inequality holds
\[\ell(i,\values, \EFone(i,\values)) \geq \ell(i,\values, \EFone(i,\values')).\]
\end{lemma}
\begin{proof}
Let $\Alloc = (A_1, A_2, \ldots, A_n) \in \EFone(i,\values)$ be an allocation such $\values(A_i) = \ell(i,\values, \EFone(i,\values))$, i.e. $\Alloc$ is the worst-case outcome for agent $i$ when her valuation vector is $\values$. If $\Alloc \in \EFone(i,\values')$, the lemma immediately follows, since the allocation $\Alloc'$ that minimizes $\values(A'_i)$ over all allocations in $\EFone(i,\values')$ could only be smaller than $\values(A_i)$. Therefore, assume without loss of generality that $\Alloc \notin \EFone(i,\values')$. We will construct an allocation $\Alloc'$ with the following properties: $(i)$ $\values(A'_i) \leq \values(A_i)$, and $(ii)$ $\Alloc' \in \EFone(i,\values')$. These two properties together imply the desired inequality, since
$\ell(i,\values,\EFone(i,\values)) = \values(A_i) \geq \values(A'_i) \geq \ell(i,\values,\EFone(i,\values'))$, where the first inequality follows from $(i)$ and the second inequality follows from $(ii)$.


Let $S^* \subseteq \agents \setminus \{i\}$ be the subset of agents with non-empty bundles in $\Alloc$, i.e., $S^* \coloneqq \{j \in \agents \setminus \{i\} \ | \ A_j \neq \emptyset \}$. Define agent $j^* \coloneqq \argmax_{k \in S^*} \min_{g \in A_k} \values'(A_k \setminus \{g\})$, to be the agent in $S^*$ whose allocation ``up to one item'' has maximum value with respect to $\values'$, and let $g^* = \argmin_{g \in A_{j^*}} \values'(A_{j^*} \setminus \{g\})$ be the favorite good with respect to $\values'$ that $j^*$ has. Given these definitions, $\Alloc'$ is defined as follows. $A'_i = A_{j^*} \setminus \{g^*\}$, $A'_{j^*} = A_i \cup \{g^*\}$, and for all agents $k \in \agents \setminus \{i,j^*\}$ we have $A'_k = A_k$. It remains to show that $\Alloc'$ satisfies $(i)$ and $(ii)$.

Towards proving $(i)$ we have $\values(A'_i) = \values(A_{j^*} \setminus \{g^*\}) \leq \values(A_i)$, where the last inequality follows from the fact that $\Alloc \in \EFone(i,\values)$.

Towards proving $(ii)$, note that $\agents \setminus \{i\}$ can be written as the union of three disjoint sets $S_1$, $S_2$ and $S_3$, where $S_1 = \agents \setminus (S^* \cup \{i\})$, $S_2 = (S^* \setminus \{j^*\})$, and  $S_3 = \{j^*\}$. We will show that in allocation $\Alloc'$ agent $i$ with valuation vector $\values'$, does not envy, up to one item, any of the agents in $S_1$, $S_2$, or $S_3$; this establishes that $\Alloc' \in \EFone(i,\values')$.
First, for every agent $k \in S_1$ we have that $A'_k = A_k = \emptyset$, by the definition of $S^*$, so agent $i$ cannot envy any such agent.
Second, given the definition of agent $j^*$, we know that for each agent $k$ in $S_2 = S^* \setminus \{j^*\}$, we have
\begin{align*}
\min_{g \in A'_k} \values'(A'_k \setminus \{g\}) & = \min_{g \in A_k} \values'(A_k \setminus \{g\}) \tag{$A'_k = A_k$ for all agents except $i$ and $j^*$}\\
& \leq \min_{g \in A_{j^*}} \values'(A_{j^*} \setminus \{g\}) \tag{by the definition of $j^*$} \\
& \leq \values'(A_{j^*} \setminus \{g^*\}) \tag{$g^* \in A_{j^*}$}\\
& = \values'(A'_i). \tag{$A'_i = A_{j^*} \setminus \{g^*\}$}
\end{align*}

Therefore, agent $i$ with valuation $\values'$ does not envy up to one item (and, in fact, up to any item) any agent in $S_2$.

Third, recall that $\Alloc \notin \EFone(i,\values')$. By definition, agent $j^*$ has the bundle that $\values'$ likes the most ``up to one item'', and $g^*$ is that most valuable (in terms of marginal value) item in $j^*$'s bundle, so $\values'(A_i) < \values'(A_{j^*} \setminus \{g^*\})$. Therefore, we have
\begin{align*}
    \values'(A'_i) & = \values'(A_j \setminus \{g^*\}) \tag{$A'_i = A_j \setminus \{g^*\}$} \\
    & > \values'(A_i) \tag{$\Alloc \notin \EFone(i,\values')$} \\
    & = \values'(A_i \cup \{g^*\} \setminus \{g^*\}) \\
    & = \values'(A'_{j^*} \setminus \{g^*\}) \tag{$A'_{j^*} = A_i \cup \{g^*\}$}.
\end{align*}
That is, agent $i$ with valuation $\values'$ does not envy, up to one item, any agent in $S_3 = \{ j^* \}$. 

This establishes that $\Alloc' \in \EFone(i,v')$ and concludes the proof.
\end{proof}

Given the previous lemmas, we can show our main theorem with respect to not obviously manipulability.

\begin{theorem}\label{thm: EF1 implies NOM}
If agents' valuation functions are monotone and $\mathcal{M}^*$ is $\EFone$, then Mechanism~\ref{mechanism:NOM+PO+EF1} is not obviously manipulable.
\end{theorem}

\begin{proof}
We first show that agents cannot improve their worst-case utilities by misreporting.

Let $i \in \agents$ be an agent whose true valuation is $\values_i$ and let her misreport be $\bids_i$. By Lemma~\ref{lemma:every-EF1-realized}, for every reported valuation vector $\bids$ of agent $i$, 
and for every allocation $\Alloc \in \EFone(i,\bids)$, there exists a valuation profile $\values_{-i}$ such that $\Alloc$ is the output of Mechanism~\ref{mechanism:NOM+PO+EF1}.
On the other hand, Mechanism~\ref{mechanism:NOM+PO+EF1} always outputs allocations $\Alloc$ that are (1) clean (by Line~\ref{code:removal}), and (2) envy free up to one item (Lemma~\ref{lemma:mech is EF1}). That is, every output allocation of Mechanism~\ref{mechanism:NOM+PO+EF1} is in $\EFone(i,\bids)$.
Therefore, if agent $i$ reports $\values_i$ (respectively $\bids_i$), then the set of all possible allocations of Mechanism~\ref{mechanism:NOM+PO+EF1} is exactly $\EFone(i,\values_i)$ (respectively $\EFone(i,\bids_i)$).
Overloading notation, let $A^*_i(\values_i, \values_{-i})$ be the allocation of agent $i$ in Mechanism~\ref{mechanism:NOM+PO+EF1}, on input $(\values_i, \values_{-i})$.
For the worst-case utility of agent $i$ we have
\begin{align*}
    \min\limits_{\values_{-i}} \values_i( A^*_i(\values_i, \values_{-i})  )& = \min\limits_{ \Alloc \in \EFone(i,\values_i)} \values_i(A_i)\\
    & = \ell(i, \values_i, \EFone(i,\values_i)) \tag{by definition} \\
    & \geq \ell(i, \values_i, \EFone(i, \bids_i)) \tag{Lemma \ref{lemma:least-valued-EF1}}\\
    & = \min\limits_{\values_{-i}} \values_i( A^*_i(\bids_i, \values_{-i})  ).
\end{align*}

This establishes Inequality~\ref{inequality:NOM-worst-case} from the definition of NOM. To conclude the proof, it remains to show that the best-case utility of an agent is also not improved by misreporting. Note that the best case for agent $i \in \agents$ occurs when all other agents have no value for the items, i.e. $D_j = \emptyset$ for all $j \in \agents \setminus \{i\}$. Hence the sets $\{D_k\}_{k \in [n]}$ are pairwise-disjoint, and Mechanism~\ref{mechanism:NOM+PO+EF1} (via \emph{Case \rm{I}}) allocates the entirety of $D_i$ to agent $i$, which is impossible to improve upon.
\end{proof}



%Now we are ready to prove the main result of this section, Theorem %\ref{theorem:NOM+PO+EF1}.

%\begin{proof}[Proof of Theorem \ref{theorem:NOM+PO+EF1}]

%\end{proof}

%Given that the mechanism $\widehat{M}$ outputs $\PO + \EFone$ allocations, if the above defined property holds, the following corollary follows.
%
%\begin{corollary}
%The worst case utility for an agent $i$ (as per her true valuation $v^t_i$), if she report her valuation to be $v_i$ is exactly $l(i,v^t_i, \EFone(i,v_i))$.
%\end{corollary}
%Note that, the mechanism $\widehat{M}$ yields $\PO$ allocations, therefore for each agent, her best-case utility under truthful reporting cannot be improved. Given this, the following lemma follows
%
%\begin{lemma}
%If for each agent $i \in [n]$ and every valuation $v_i \in \mathbb{R}^m_{\geq 0}$, the following inequality is true
%\begin{align*}
%l(i,v^t_i, \EFone(i,v^t_i)) \geq l(i,v^t_i, \EFone(i,v_i)),
%\end{align*}
%then the mechanism $\widehat{M}$, which outputs $\PO + \EFone$ allocations, is $\NOM$.
%\end{lemma}


\subsection{Ex-ante EF, Ex-post fPO, Ex-post EF1 and NOM}

In the previous section we established (Application~\ref{application: additive}) the existence of a deterministic NOM mechanism that outputs ex-post fPO and EF1 allocations for additive agents. Here we make a short remark that it is not possible to improve upon this result by adding ex-ante fairness guarantees. Specifically, there does not exist a randomized mechanism that is NOM in expectation and outputs ex-post fPO and EF1 allocations, that is additionally ex-ante envy-free. This follows directly from the following impossibility result of~\citet{freeman2020best}.

\begin{theorem}[\cite{freeman2020best}]
There exists instances with additive valuation where there is no randomized allocation that is simultaneously ex-post fPO and $\EFone$, and ex-ante envy-free.
\end{theorem}


==> intro_old.tex <==
\section{Introduction}\label{sec: intro}

We consider the fundamental problem of allocating a set of indivisible items among strategic agents.
Even for the case of two additive agents, it is well-understood that, in the absence of monetary transfers, fairness, efficiency and truthfulness cannot be reconciled, in a very strong sense.
For example, a serial dictatorship (arguably the most unfair allocation rule) is the \emph{unique} truthful and Pareto efficient mechanism~\cite{papai2000strategyproof, klaus2002strategy, ehlers2003coalitional}, even for the case of two additive agents and randomized mechanisms (or, equivalently, divisible items)~\cite{schummer1996strategy}. At the same time, achieving envy-freeness up to one item (EF1)~\cite{budish2011combinatorial}, one of the most popular fairness notions for indivisible goods that is compatible with Pareto efficiency\cite{caragiannis2019unreasonable}, is impossible for truthful and deterministic mechanisms to achieve, even for two additive agents~\cite{amanatidis2017truthful}.

The standard treatment of a strategic agent is to assume that, when presented with an algorithm, the agent will perfectly understand it and optimally respond to it. Therefore, a truthful mechanism should protect against all deviating strategies. In this paper we aim to escape the aforementioned impossibility results for truthful mechanisms by relaxing this requirement: our goal is to design mechanisms that protect only against \emph{obviously dominant} deviating strategies. 

Informally, a strategy is obviously dominant if it guarantees an outcome better than any outcome of every other strategy~\cite{li2017obviously}. Designing obviously truthful mechanisms, those where honest reporting is obviously dominant, is a problem that has attracted significant attention in the past few years~\cite{ashlagi2018stable,kyropoulou2019obviously,ferraioli2019obvious,arribillaga2020obvious}. However, since dishonesty is also a strategy, a deviation can be profitable but not obviously profitable. A manipulation is obvious if it yields a higher utility than truth-telling in either the best or worst-case scenarios. Seminal work of~\citet{troyan2020obvious} defines this notion, and shows that relaxing truthfulness to non-obvious manipulability can strictly improve the designer's objective in a number of domains (e.g. two-sided matching).

In this paper we aim to provide a comprehensive study of what can and what cannot be achieved by non-obviously manipulable mechanisms in the fundamental problem of fair and efficient allocation of indivisible goods.

\subsection{Our Contribution}


We first consider the problem of designing a non-obviously manipulable mechanism (NOM) which always outputs allocations that are envy-free up to one item (EF1), a task that is impossible for truthful mechanisms to achieve~\cite{amanatidis2017truthful}. We prove that the Round-Robin procedure (agents choose items one at a time, following a fixed order) which is known to always output EF1 allocations, is also not obviously manipulable (Theorem~\ref{thm:rr is nom}), giving a separation between truthfulness and non-obviously manipulability for our problem. In fact, we show that NOM is compatible with even stronger notions of fairness. Specifically, a fairness guarantee stronger than EF1 that a randomized algorithm could satisfy is to be ex-post EF1 (i.e. to always output an EF1 allocation), and simultaneously be envy-free in expectation (ex-ante). There are known algorithms that satisfy this ``best-of-both-worlds'' guarantee~\cite{freeman2020best,aziz2020simultaneously}; we show that the PS-Lottery algorithm of~\cite{aziz2020simultaneously} is not-obviously manipulable. This result uses a connection between ex-ante proportionality and not obvious manipulability; we later exploit this connection to give new negative ``best-of-both-worlds'' results!


We proceed to study efficient algorithms. Specifically, we study the three most common notions of efficiency in this setting: utilitarian social welfare (the sum of agents' utilities), egalitarian social welfare (the minimum of agents' utilities), and Nash social welfare (the geometric mean of agents' utilities). For the case of $n=2$ additive agents all three notions are incompatible with non obvious manipulability, i.e. every (deterministic or randomized) algorithm that always outputs an integral solution that is optimal with respect to any of these objectives is obviously manipulable (Theorem~\ref{theorem:NOM+SWM+2agents}). This is also true for the case of more than three agents for egalitarian and Nash social welfare (Theorems~\ref{thm: NOM + egalitarian + n agents} and~\ref{thm: MNW impossibility}).
The intuition for these impossibilities is the following. There are instances where a specific agent\footnote{Informally, the agent that the tie-breaking rule favors.} gets her least favorite item, in the worst-case. However, solutions that are optimal for egalitarian and Nash welfare prioritize maximizing the number of agents that get non-zero utility. Therefore, by reporting that she only values a single item (her favorite item) to the mechanism, this agent can force the mechanism to give her this item (or increase the probability that she gets it) in the worst-case.
Surprisingly, the same is not true for utilitarian social welfare:\footnote{Note that when discussing utilitarian social welfare, we assume that the input is normalized, i.e. the utility of an agent for the grand bundle of items is equal to $1$. See Section~\ref{sec: efficient} for details.} there is a not-obviously manipulable algorithm that always outputs an allocation that maximizes utilitarian social welfare for the case of $n \geq 3$ additive agents (Theorem~\ref{theorem:NOM+SWM+nagents}). This gives an efficient and not obviously manipulable mechanism that is not dictatorial.
%Therefore, in contrast to truthfulness~\cite{klaus2002strategy,schummer1996strategy}, there are non-dictatorial mechanisms that are not obviously manipulable and efficient.

Since maximizing Nash social welfare, a common way to simultaneously achieve Pareto efficiency and envy-freeness up to one item, is obviously manipulable, the next natural question is whether there are any other Pareto efficient and EF1 algorithms that are not-obviously manipulable, for the case of additive agents. Our main result answers this question in the affirmative. In fact, we prove that the problem of designing a Pareto efficient, EF1 and NOM \emph{mechanism} is exactly as hard as designing a Pareto efficient and EF1 \emph{algorithm}. We give a black-box reduction that (approximately) preserves Pareto efficiency guarantees, which given an algorithm that always outputs EF1 allocations, outputs a mechanism that is not obviously manipulable and always outputs EF1 allocations, even for agents with general monotone valuations.
Intuitively, there are two crucial steps in our reduction. Given the valuation function $\values_i$ of agent $i$, let $\EFone(i,\values_i)$ be the set of allocations that are clean\footnote{A set of items $S$ is clean for agent $i$ if the removal of any good reduces $i$'s value for $s$  $\values_i(S) > \values_i (S \setminus \{ g \} )$ for all $g \in S$.} and $\EFone$ for agent $i$. %, i.e. $\EFone(i,\values_i) = \{ \Alloc \in \Pi_n(\items) \ | \forall g \in A_i ~~ \values_i(A_i \setminus \{ g \} ) < \values_i(A_i), \text{ and } \forall j \in \agents \text{ with } A_j \neq \emptyset, \values_i(A_i) \geq \values_i(A_j \setminus \{g\}) \text{ for some }g \in A_j\}$. 
First, our reduction ensures that, when agent $i$ considers a reporting her valuation as $\bids_i$, every single allocation in $\EFone(i,\bids_i)$ is possible, i.e. for every allocation $\Alloc \in \EFone(i,\bids_i)$ there are reports for the other agents such that $\Alloc$ is the output of the mechanism. Second, we prove the following intuitive structural result, that might be of independent interest. For agent $i$ with a monotone valuation function $\values_i$, the worst-case allocation in $\EFone(i,\values_i)$ is better than the worst-case allocation in $\EFone(i,\bids_i)$ (Lemma~\ref{lemma:least-valued-EF1}). These facts combined give the ``worst-case'' part from the definition of NOM, which is the most challenging step. Direct applications of our reduction, by giving as input known algorithmic results~\cite{garg2021improved,chaudhury2021fair,lipton2003playing}, we get (1) an EF1 and NOM mechanism for the case of monotone agents, (2) an EF1, approximately efficient and NOM mechanism for the case of subadditive agents, and (3) an fPO, EF1 and NOM mechanism for additive agents; this last result cannot be improved by adding ex-ante fairness guarantees (due to a result of~\cite{freeman2020best}).

Overall, our results show a connection between certain notions of fairness and not obvious manipulability: positive algorithmic results for $\EFone$ and ``best-of-both-worlds'' guarantees can be used to get positive results for not obviously manipulable mechanisms. In Section~\ref{sec: best of both} we exploit this connection in the other direction, and show how negative results for not obviously manipulable mechanisms can be used to give new negative results for ``best-of-both-worlds'' algorithms. 
Specifically, we prove that for the case of additive valuations, it is impossible to achieve ex-ante proportionality, ex-post Pareto efficiency while ex-post maximizing the number of agents with positive utility. As direct corollaries we recover a known result of~\citet{freeman2020best} that ex-ante proportional and ex-post MNW allocations do not exist, as well as two new results: it is impossible to (always) achieve ex-ante proportionality by randomizing over allocations that are (1) ex-post Pareto efficiency and ex-post egalitarian, or (2) ex-post leximin.


\subsection{Related work}

%Obvious strategy-proofness, recently proposed by~\citet{li2017obviously}, is a paradigm that attempts to explain the prevalence of some auction formats over others (e.g. ascending auctions versus sealed-bid second price auctions). This definition has become increasingly popular, with many recent works study obvious strategyproof mechanisms.
\citet{troyan2020obvious} define the notion of not obvious manipulability. They show that a number of known mechanisms which are not strategyproof satisfy not obviously manipulability, e.g. stable mechanisms in the context of two-sided matching are not obviously manipulable (in direct contrast to~\citet{roth1982economics}, who shows that there exists no mechanism that is both stable and strategyproof). At the same time, many known not strategyproof mechanisms are obviously manipulable, e.g. the first-price auction, and more generally the pay-as-bid auction.



%In the context of \alex{one-sided matching?}, they show that the Boston mechanism is obviously manipulable, while stable-dominating mechanisms are not obviously manipulable. In the context of two-sided matching they show that any stable mechanism is individually rational, Pareto efficient, and not obviously manipulable, in direct contrast to~\citet{roth1982economics} who shows that there exists no mechanism that is both stable and strategy-proof. In the contexts of auctions, they show that the first price auction (and more generally the pay-as-bid auction) is obviously manipulable, while the $(K+1)$-price auction (for $K=1$ this is the second price auction) is not obviously manipulable. For bilateral trade, the double auction mechanism is obviously manipulable, while every efficient, individually rational, and weakly budget balanced mechanism is obviously manipulable.

The notion of non obvious manipulability in computational social choice has been explored in some very recent works~\cite{ortega2019obvious,aziz2021obvious}.~\citet{ortega2019obvious} study cake-cutting. They show that, as opposed to truthfulness, NOM is compatible with proportionality: an adaptation of the well-known moving knife procedure satisfies both properties. They also observe that every proportional (direct revelation) rule satisfies the worst-case guarantee required for NOM (we show a similar statement here, in Lemma~\ref{lemma:ex-ante-EF-and-NOM}), while every Pareto efficient (direct revelation) rule satisfies the best-case guarantee required for NOM. Therefore, in the context of direct revelation mechanisms in cake-cutting, proportional and Pareto efficient rules are not obviously manipulable. \citet{aziz2021obvious} explore obvious manipulations in voting theory. They give sufficient conditions for voting rules to be not obviously manipulable, and show that a number of voting rules escape the pessimistic conclusions of the Gibbard-Satterthwaite theorem, e.g., the Borda rule is not obviously manipulable.


%\alex{other relaxations of IC}
%\cite{bartholdi1989computational}


Other than relaxing the notion of incentive compatibility, one can escape the aforementioned impossibility results for no-money truthful mechanisms by restricting agents' valuations, e.g. focus on dichotomous~\cite{halpern2020fair,babaioff2021fair,benabbou2021finding,barman2021truthful} or 
Leontief valuations~\cite{ghodsi2011dominant,friedman2014strategyproof,parkes2015beyond}, or by using money-burning (wasting resources) as a substitute for payments~\cite{hartline2008optimal,cole2013mechanism,fotakis2016efficient,friedman2019fair,abebe2020truthful}.


Ignoring incentives altogether, there is a growing literature that studies the problem of allocating indivisible goods in a fair and efficient manner.
For additive agents,~\citet{caragiannis2019unreasonable} show that the integral allocation that maximizes the Nash social welfare is Pareto efficient and envy-free up to one item. Finding such allocations is APX-hard~\cite{lee2017apx}. However,~\citet{barman2018finding} give an algorithm for finding a Pareto efficient and $\EFone$ allocation that runs in pseudo-polynomial time (and polynomial time for bounded valuations) for the case of additive agents.~\citet{barman2018finding} also provide a proof of existence for $\EFone$ and fractionally Pareto efficient allocations; recent work by~\citet{garg2021fair} gives a pseudo-polynomial time algorithm for finding such allocations. Beyond additive agents,~\citet{caragiannis2019unreasonable} show that there are no Pareto efficient and $\EFone$ allocations for subadditive or supermodular valuations. And, while the problem of approximating the Nash social welfare under different valuation functions (sometimes even combined with some fairness guarantees) has received significant attention in the past few years~\cite{cole2018approximating,cole2017convex,anari2018nash,garg2018approximating,chaudhury2018fair,chaudhury2021fair,chaudhury2021little}, to the best of our knowledge the
existence of Pareto efficient and $\EFone$ allocations, even for submodular valuations, remains open. However, we do note that, if such allocations exist (or even $\EFone$ and approximately-Pareto  efficient allocations exist), our main result (Theorem~\ref{theorem:NOM+PO+EF1}) implies that there also exists a NOM mechanism with the same guarantee.
%Finally, we note that there are other, extensively studied, notions of fairness for indivisible goods, notably the max-min share (MMS) guarantee~\cite{budish2011combinatorial,bouveret2016characterizing,amanatidis2017approximation,barman2020approximation,kurokawa2018fair,ghodsi2018fair,garg2018approximating,garg2021improved}.







==> macros.tex <==
\usepackage[numbers]{natbib}
\usepackage{xspace}
\usepackage[margin=1in]{geometry}
\usepackage{pstricks}
\usepackage{comment}
\usepackage{dsfont}
\usepackage{tikz}
\usepackage{tikz-dependency}
\usepackage{mathrsfs}
\usepackage{appendix}

\usepackage{amsmath,amssymb,amsthm,amsfonts,latexsym,bbm,xspace,graphicx,float,mathtools,mathdots}
\usepackage{braket,caption,subcaption,ellipsis,xcolor,textcomp}
\usepackage[colorlinks,citecolor=blue]{hyperref}
\usepackage[margin=1in]{geometry}
\usepackage{enumerate}
\usepackage{enumitem}
\usepackage[ruled]{algorithm2e}
\IncMargin{-\parindent}
\usepackage{algpseudocode}
\usepackage{listings}
\usepackage{algcompatible}
\usepackage{float}
\floatstyle{ruled}

% Restating theorems
\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{cleveref}
%\usepackage[protrusion=true,expansion=true]{microtype}   % slows compilation a lot

%\usepackage[colorinlistoftodos]{todonotes}               % so slow
\usepackage[colorinlistoftodos,disable]{todonotes}

\def\showauthnotes{1}

\ifthenelse{\showauthnotes=1}
{
%\newcommand{\authnote}[2]{{ \footnotesize \bf{[#1: #2]~}}}
\newcommand{\authnote}[2]{[{\color{blue}\textbf{#1:}}~{\color{blue} #2}]}
}
{ \newcommand{\authnote}[2]{} 
}
\newcommand{\alex}[1]{\authnote{Alex}{#1}}
\newcommand{\paritosh}[1]{\authnote{Paritosh}{#1}}


\usepackage{accents}
\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
\newcommand{\alloc}{\mathbf{x}}
\newcommand{\ralloc}{\mathbf{r}}
\newcommand{\allocy}{\mathbf{y}}
\newcommand{\allocz}{\mathbf{z}}
\newcommand{\bids}{\mathbf{b}}
\newcommand{\values}{\mathbf{v}}
\newcommand{\items}{\mathrm{M}}
\newcommand{\agents}{\mathrm{N}}
\newcommand{\vmin}{\epsilon}

%----Fair Division Terms----
\newcommand{\NOM}{\textsc{NOM}}
\newcommand{\PO}{\textsc{PO}}
\newcommand{\fPO}{\mathrm{fPO}}
\newcommand{\EFone}{\mathrm{EF}1}
\newcommand{\Alloc}{\mathcal{A}}
\newcommand{\SW}{\textsc{SW}}
\newcommand{\NSW}{\textsc{NSW}}
\newcommand{\MNW}{\textsc{MNW}}
\newcommand{\ESW}{\textsc{ESW}}

% environments
\newtheorem{theorem}{Theorem}
\declaretheorem[name=Theorem,sibling=theorem]{thm-restate}
% See https://tex.stackexchange.com/questions/51286/recalling-a-theorem for usage

\newtheorem{lemma}{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{proposition}{Proposition}
\newtheorem{fact}{Fact}
\newtheorem{corollary}{Corollary}
\newtheorem{conjecture}{Conjecture}
\newtheorem{question}{Question}
\newtheorem{answer}{Answer}
\newtheorem{hypothesis}{Hypothesis}
\newtheorem{problem}{Problem}
\newtheorem{observation}{Observation}

\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newtheorem{notation}{Notation}
\newtheorem{example}{Example}
\newtheorem{examples}{Example}
\newtheorem{algo}{Algorithm}
\newtheorem{rgoal}{Research Goal}
\newtheorem{egoal}{Educational Goal}


% probability and other mathops
\renewcommand{\Pr}{\mathop{\bf Pr\/}}
\newcommand{\E}{\mathop{\bf E\/}}
\newcommand{\Ex}{\mathop{\bf E\/}}
\newcommand{\Var}{\mathop{\bf Var\/}}
\newcommand{\Cov}{\mathop{\bf Cov\/}}
\newcommand{\stddev}{\mathop{\bf stddev\/}}
\newcommand{\littlesum}{\mathop{{\textstyle \sum}}}
\newcommand{\littleprod}{\mathop{{\textstyle \prod}}}
\newcommand{\Opt}{\textnormal{OPT\/}}
\newcommand{\Alg}{\textnormal{ALG\/}}
\newcommand{\Cost}{\mathop{ Cost\/}}

% math terms
\newcommand{\poly}{\textnormal{poly}}
\newcommand{\polylog}{\textnormal{polylog}}
\newcommand{\size}{\textnormal{size}}
\newcommand{\avg}{\mathop{\textnormal{avg}}}
\newcommand{\sgn}{\textnormal{sgn}}
\newcommand{\dist}{\textnormal{dist}}
\newcommand{\vol}{\textnormal{vol}}
\newcommand{\spn}{\textnormal{span}}
\newcommand{\supp}{\textnormal{supp}}
\newcommand{\codim}{\operatorname{codim}}
\newcommand{\rank}{\textnormal{rank}}
\newcommand{\nullity}{\textnormal{nul}}
\newcommand{\trace}{\textnormal{trace}}

% number systems
\newcommand{\R}{\mathbbm R}
\newcommand{\C}{\mathbbm C}
\newcommand{\N}{\mathbbm N}
\newcommand{\Z}{\mathbbm Z}
\newcommand{\F}{\mathbbm F}
\newcommand{\Q}{\mathbbm Q}

% complexity classes
\newcommand{\PTIME}{\mathsf{P}}
\newcommand{\LOGSPACE}{\mathsf{L}}
\newcommand{\ZPP}{\mathsf{ZPP}}
\newcommand{\RP}{\mathsf{RP}}
\newcommand{\CORP}{\mathsf{CoRP}}
\newcommand{\BPP}{\mathsf{BPP}}
\newcommand{\NP}{\mathsf{NP}}
\newcommand{\CONP}{\mathsf{CoNP}}
\newcommand{\TC}{\mathsf{TC}}
\newcommand{\AC}{\mathsf{AC}}
\newcommand{\SC}{\mathsf{SC}}
\newcommand{\SZK}{\mathsf{SZK}}
\newcommand{\MA}{\mathsf{MA}}
\newcommand{\AM}{\mathsf{AM}}
\newcommand{\IP}{\mathsf{IP}}
\newcommand{\PSPACE}{\mathsf{PSPACE}}
\newcommand{\EXP}{\mathsf{EXP}}
\newcommand{\ETIME}{\mathsf{E}}
\newcommand{\MIP}{\mathsf{MIP}}
\newcommand{\NEXP}{\mathsf{NEXP}}
\newcommand{\BQP}{\mathsf{BQP}}
\newcommand{\TIME}{\mathsf{TIME}}
\newcommand{\PP}{\mathsf{PP}}
\newcommand{\PPOLY}{\mathsf{P}/\mathsf{poly}}
\newcommand{\PH}{\mathsf{PH}}
\newcommand{\SPACE}{\mathsf{SPACE}}
\newcommand{\DTIME}{\mathsf{DTIME}}
\newcommand{\NTIME}{\mathsf{NTIME}}
\newcommand{\SHARPP}{\#\PTIME}
\newcommand{\ACC}{\mathsf{ACC}}
\newcommand{\SYMPLUS}{\mathsf{SYM+}}
% short forms
\newcommand{\eps}{\epsilon}
\newcommand{\lam}{\lambda}
\newcommand{\dleta}{\delta}
\newcommand{\vphi}{\varphi}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\ot}{\otimes}
\newcommand{\zo}{\{0,1\}}
\newcommand{\co}{:}                       %\newcommand{\co}{\colon}
\newcommand{\bdry}{\partial}
\newcommand{\grad}{\nabla}
\newcommand{\symmdiff}{\triangle} \newcommand{\symdiff}{\symmdiff}
\newcommand{\half}{\tfrac{1}{2}}

% calligraphic letters
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}

% bold
\newcommand{\bone}{\boldsymbol{1}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bvphi}{\boldsymbol{\varphi}}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\ba}{\boldsymbol{a}}
\newcommand{\bb}{\boldsymbol{b}}
\newcommand{\bc}{\boldsymbol{c}}
\newcommand{\bd}{\boldsymbol{d}}
\newcommand{\be}{\boldsymbol{e}}
\newcommand{\boldf}{\boldsymbol{f}}
\newcommand{\bg}{\boldsymbol{g}}
\newcommand{\bh}{\boldsymbol{h}}
\newcommand{\bi}{\boldsymbol{i}}
\newcommand{\bj}{\boldsymbol{j}}
\newcommand{\bk}{\boldsymbol{k}}
\newcommand{\bell}{\boldsymbol{\ell}}
\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\bt}{\boldsymbol{t}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\bx}{{\boldsymbol{x}}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\bA}{\boldsymbol{A}}
\newcommand{\bB}{\boldsymbol{B}}
\newcommand{\bC}{\boldsymbol{C}}
\newcommand{\bD}{\boldsymbol{D}}
\newcommand{\bE}{\boldsymbol{E}}
\newcommand{\bF}{\boldsymbol{F}}
\newcommand{\bG}{\boldsymbol{G}}
\newcommand{\bH}{\boldsymbol{H}}
\newcommand{\bI}{\boldsymbol{I}}
\newcommand{\bJ}{\boldsymbol{J}}
\newcommand{\bL}{\boldsymbol{L}}
\newcommand{\bP}{\boldsymbol{P}}
\newcommand{\bR}{\boldsymbol{R}}
\newcommand{\bS}{\boldsymbol{S}}
\newcommand{\bT}{\boldsymbol{T}}
\newcommand{\bU}{\boldsymbol{U}}
\newcommand{\bV}{\boldsymbol{V}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bZ}{\boldsymbol{Z}}

% left-right wrappers
\DeclarePairedDelimiter\parens{\lparen}{\rparen}
\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\braces{\lbrace}{\rbrace}
\DeclarePairedDelimiter\bracks{\lbrack}{\rbrack}
\DeclarePairedDelimiter\angles{\langle}{\rangle}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}


%%%%%%%%%%%%% hyphenation %%%%%%%%%%%%%

\hyphenation{Naka-shima}

%%%%%%%%%%%%% 10701 %%%%%%%%%%%%%%%%%%%%
\newcommand{\normsq}[1]{\norm*{#1}^2}


